Efficient and Deployable Knowledge Infusion for Open-World Recommendations via Large Language Models

Recommender systems (RSs) play a pervasive role in today's online services, yet their closed-loop nature constrains their access to open-world knowledge. Recently, large language models (LLMs) have shown promise in bridging this gap. However, previous attempts to directly implement LLMs as recommenders fall short in meeting the requirements of industrial RSs, particularly in terms of online inference latency and offline resource efficiency. Thus, we propose REKI to acquire two types of external knowledge about users and items from LLMs. Specifically, we introduce factorization prompting to elicit accurate knowledge reasoning on user preferences and items. We develop individual knowledge extraction and collective knowledge extraction tailored for different scales of scenarios, effectively reducing offline resource consumption. Subsequently, generated knowledge undergoes efficient transformation and condensation into augmented vectors through a hybridized expert-integrated network, ensuring compatibility. The obtained vectors can then be used to enhance any conventional recommendation model. We also ensure efficient inference by preprocessing and prestoring the knowledge from LLMs. Experiments demonstrate that REKI outperforms state-of-the-art baselines and is compatible with lots of recommendation algorithms and tasks. Now, REKI has been deployed to Huawei's news and music recommendation platforms and gained a 7% and 1.99% improvement during the online A/B test.

==> backup.tex <==
\section{Introduction}
% recommender system are closed systems, lack world knowledge
% capability of large lanugage models: reasoning and world knowledge; black box and white box llm; Adopting llm for rec as in existing methods [xxx] is infeasible: a) lack rec domain knowledge, cannot fast inference according to ever-changing user behavior data; b) require extreme large computational resource to train the model.

% fully exploit reasoning and world knowledge of llm as well as domain knowledge, while keep efficient inference.
% challenge: the utilization of llm to recsys: a) text/super large dense vector b) noise information c) in syntactic and recommendation space are not aligned (unisrec).


 % Dai \textit{et al.}~\cite{dai2023uncovering} analyze the recommendation ability of ChatGPT in terms of point-wise, pair-wise, and list-wise tasks. 
 % LLMs are not designed to capture the delicate interaction patterns between user and item features. 

% providing dynamic response and personalization to users. These 



% The emergence of LLMs has brought about a paradigm shift in
% research.

% shown  With the immense scale of the model and the corpus size, large language models (LLMs) 

% representations and encode extensive world knowledge
% , and allows the recommender systems to provide human-like recommendations with clear evidence.
% (\eg, the user's clicked, purchased items)

% uncover the underlying motives and correlations between the behaviors and the contexts, enabling a more comprehensive understanding of the users. Seasonal factors or external events for temporal preference deduction. For instance, . These preference reasoning goes beyond identifying basic behavior patterns as in classical recommender systems, and help the recommender systems comprehend the underlying motives and correlations between the behaviors and the contexts.

% users bought textbooks imply that they may be college students; users bought ski boots imply that they may be interested in outdoor activities
% Yet user behaviors are complex
% given the user behavior history (\eg, the user's clicked, purchased items), one can analyze and infer the personalized preferences and intentions, which is intrinsically a multi-step reasoning problem. For instance, a user bought a 

% On the one hand, integrating external information about the users and the items enables a more comprehensive understanding of the recommendation task. On the other hand, by applying logical reasoning to user behavior history, recommender systems can analyze the underlying motives and correlations between the behaviors and the contexts, and can even integrate seasonal factors or external events for temporal preference deduction. This kind of preference reasoning goes beyond identifying basic behavior patterns as in classical recommender systems, and is more similar to the actual reasoning process of a \textit{human}.

% It helps us understand
% the "why" behind user preferences and enables more accurate and
% personalized recommendations

% the \textit{direct knowledge} on users and items, and the \textit{logical reasoning} on user preferences. On the one hand, integrating external information about the users and the items enables a more comprehensive understanding of the recommendation task. On the other hand, by applying logical reasoning to user behavior history, recommender systems can analyze the underlying motives and correlations between the behaviors and the contexts, and can even integrate seasonal factors or external events for temporal preference deduction. This kind of preference reasoning goes beyond identifying basic behavior patterns as in classical recommender systems, and is more similar to the actual reasoning process of a \textit{human} performing recommendation.


Recommender systems (RSs) are ubiquitous in today's online services, shaping and enhancing user experiences in various domains such as movie discovery~\cite{koren2009matrix}, online shopping~\cite{he2016ups}, and music streaming~\cite{van2013deep}. However, a common characteristic of existing recommender systems is their  \textit{insulated nature} --- the models are trained and deployed within closed systems. As depicted in Figure~\ref{fig:intro}(a), the data utilized in a classical recommender system is confined to one or a few specific application domains~\cite{koren2009matrix, DIN}, isolated from the knowledge of the external world, thereby restricting the information that could be learned for a recommendation model. In fact, knowledge beyond the given domains can significantly enhance the predictive accuracy and the generalization ability of recommender systems~\cite{friedman2023leveraging,lin2023sparks}. Hence, in this work, we posit that instead of solely learning from narrowly defined data in the \textbf{closed systems}, recommender systems should be the \textbf{open-world systems} that can proactively acquire knowledge from the external world, as shown in Figure~\ref{fig:intro}(b).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{imgs/open-world-rec.pdf}
    % \caption{Comparison between closed recommender systems and open-world recommender systems. (a) Closed recommender systems. (b) Open-world recommender systems.
    % \vspace{-20pt}
    \caption{Comparison between (a) closed recommender systems and (b) open-world recommender systems.}
    % \vspace{-15pt}
    % \Jianghao{Comparison between (a) closed recommender systems and (b) open-world recommender systems.}}
    \label{fig:intro}
\end{figure}

In particular, some knowledge from the external world is especially useful for recommendation, which we refer to as \textit{open-world knowledge} for recommendation, including the factual knowledge on items that can be directly obtained from the web, and user-side knowledge about in-depth user preferences which is reasoned from user behaviors and profiles. On the one hand, the factual knowledge of items provides valuable common sense information about the candidate items, thereby improving the recommendation quality. Take movie recommendation as an example, the external world contains additional movie features such as \textit{plots, related reports, awards, critic reviews} that have not been included in the recommendation dataset, which expands the original data and is beneficial to the recommendation task. On the other hand, the user-side knowledge inferred from the user behavior history enables a more comprehensive understanding of the users, and is critical for better recommendation performance. Deducing the underlying preferences and motives that drive user behaviors can help us gain deeper insights and clues about the users. A person's personality, occupation, intentions, preferences, and tastes could be reflected in their behavior history~\cite{liu2023joint}.  This preference reasoning can even integrate seasonal factors (\eg, holiday-themed movie preferences during Christmas) or external events (\eg, an increased interest in health products during a pandemic) and provide human-like recommendations with clear evidence, which goes beyond identifying basic behavior patterns as in classical recommenders. 

% \cb{just for user preference reasoning? item relations reasoning?}

Several existing studies attempt to complement the closed recommender systems with additional information by knowledge graphs \cite{guo2020survey,wang2019knowledge} or multi-domain learning \cite{star,guo2023disentangled,ji2023teachers}. However, constructing comprehensive and accurate knowledge graphs or multi-domain datasets requires considerable extra human effort, and the accessible knowledge remains limited. Moreover, they only focus on extracting factual knowledge from the external world and overlook the reasoning knowledge on user preferences \cite{guo2020survey}. For instance, knowledge graphs used in RS usually focus on complement knowledge for items and rarely consider users~\cite{guo2020survey,wang2019knowledge,wang2019multi} since the user-side knowledge is highly dynamic and challenging to capture within a fixed knowledge graph.


Recent rapid developments in large language models (LLMs) have revolutionized the learning paradigm of various research fields and show great potential in bridging the gap between classical recommenders and open-world knowledge~\cite{zhao2023survey,zhu2023large,chen2023large}. With the immense scale of the model and the corpus size, these large language models like GPT-4~\cite{gpt4}, LLaMA~\cite{llama} have shown remarkable capabilities, such as problem solving, logical reasoning, creative writing~\cite{bubeck2023sparks}. Learning from an extensive corpus of internet texts, LLMs have encoded a vast array of world knowledge --- from basic factual information to complex societal norms and logical structures~\cite{bubeck2023sparks}. As a result, LLMs can perform basic logical reasoning that aligns with our known facts and relationships~\cite{wei2022chain,zhou2023leasttomost}. 



Recently, a few studies have attempted to apply LLMs as recommenders by converting recommendation tasks and user profiles into prompts~\cite{chatrec,liu2023chatgpt,dai2023uncovering}. Though some preliminary findings have been obtained, the results of directly using LLMs as recommenders are far from optimal for real-world recommendation scenarios due to the following shortcomings. 
% 1) \textbf{Predictive accuracy.} The accuracy of LLMs is generally outperformed by classical recommenders in most cases, since LLMs have not been trained on specific recommendation data~\cite{liu2023chatgpt}. The lack of recommendation domain knowledge and collaborative signals prevents LLMs from adapting to individual user preferences. 
1)~\textbf{Online Inference Latency.} To meet the real-time demands of users, industrial recommendation systems typically have strict latency requirements (usually within 100 milliseconds~\cite{DIR}). However, due to the inherent limitation of LLMs -- the excessive number of model parameters -- it is impractical to directly use LLMs as recommenders in industrial settings. With billions of users and thousands of user behaviors, LLMs fail to meet the low latency requirement. The large model size also hinders the possibility of employing real-time user feedback to update and refine the model as in classical recommenders.
2)~\textbf{Offline Resource Consumption.} Here, we refer resource to both time and computational resources. Based on existing work~\cite{bao2023tallrec,p5,lin2023rella}, the good performance of LLMs in recommendation scenarios usually entails the fine-tuning of LLMs on specific recommendation data. However, recommendation scenarios typically involve a large number of users and items, and the distribution of user behavior tends to change over time. To obtain satisfactory results on such data, it usually requires continuous fine-tuning of LLMs on regularly updated and substantial amounts of data, leading to substantial offline time and computational resource consumption.
3)~\textbf{Compositional Gap.} LLMs often suffer from the issue of compositional gap, where LLMs have difficulty in generating correct answers to the compositional problem like recommending items to users, whereas they can correctly answer all its sub-problems~\cite{press2022measuring}. Requiring direct recommendation results from LLMs is currently beyond their capability, and this approach cannot fully exploit the open-world knowledge encoded in LLMs~\cite{kang2023llms,dai2023uncovering}.

 % \Jianghao{Model complexity is also the reason why not tune LLM. I think \textbf{Inference latency} is better}

Therefore, the goal of this work is to effectively incorporate open-world knowledge from LLMs while preserving the advantages of classical recommender systems. However, despite the appealing capabilities of LLMs, extracting and utilizing knowledge from them is a non-trivial task. For one thing, LLMs encode vast corpora of world knowledge across various scenarios. Identifying proper external knowledge for recommendation and eliciting the accurate reasoning process on user preferences are quite challenging. Moreover, the world knowledge generated by LLMs is in the form of human-like texts and cannot be interpreted by recommendation algorithms. Even if some LLMs are open-sourced, the decoded outputs are usually large dense vectors (\eg, 4096 for each token), which are highly abstract and not directly compatible with recommender systems. Effectively transforming the output knowledge to be compatible with the recommendation space, without information loss or misinterpretation, is pivotal for the quality of the recommendation. Besides, the knowledge generated by LLMs can sometimes be unreliable or misleading due to the hallucination problem~\cite{ji2023survey}. More importantly, in some recommendation scenarios, the number of users and items can be enormous, even achieving a billion-level. Generating knowledge for such a large number of items and users  can be time-consuming and resource-intensive. Hence, it is critical to extract open-world knowledge from LLMs efficiently while enhancing the availability and reliability of the knowledge, to fully unleash the potential of open-world recommender systems.

To address the above problems, we propose an Open-World \underline{R}ecommendation Framework with \underline{E}fficient \underline{K}nowledge \underline{A}ugmented from Large Language Models, (dubbed \textit{REKA}). REKA is a model-agnostic framework that bridges classical recommender systems and open-world knowledge, leveraging LLMs' reasoning and factual knowledge. By first leveraging LLMs to generate open-world knowledge, and then applying classical recommender systems to model collaborative signals, we combine the advantages of both LLMs and RSs and significantly improve the model's predictive accuracy. We also propose acceleration approaches, such as the user and item clustering and prestoring the obtained knowledge, to avoid inference latency and resource efficiency issues when incorporating LLMs in RSs. 

% \cb{why not use OpenRec directly?}

Specifically, REKA consists of three stages: (1) knowledge reasoning and generation, (2) knowledge adaptation, and (3) knowledge utilization. To avoid the compositional gap for knowledge reasoning and generation, we propose \textit{factorization prompting} to break down the complex preference reasoning problem into several vital factors to generate the reasoning knowledge on users and the factual knowledge on items. With factorization prompting, we devise two distinct approaches, \textit{individual knowledge extraction} and \textit{collective knowledge extraction}, for recommendation scenarios of varying scales. In individual knowledge extraction for scenarios with limited users and items, LLMs are employed to generate individual knowledge for each user and item. Collective knowledge extraction is designed for scenarios with enormous users and items, where we first cluster items and users and then generate collective knowledge for each cluster.  Then, the knowledge adaptation stage transforms the generated knowledge into augmented vectors in the recommendation space. In this stage, we propose \textit{hybrid-expert adaptor} module to reduce dimensionality and ensemble multiple experts for robust knowledge learning, thus increasing the reliability and availability of the generated knowledge. Finally, in the knowledge utilization stage, the recommendation model incorporates the augmented vectors with original domain features for prediction, combining both the recommendation domain knowledge and the open-world knowledge. Our main contributions can be summarized as follows:
\begin{itemize}
    \item We present an open-world recommender system, REKA, which efficiently bridges the gap between the recommendation domain knowledge and the open-world knowledge from LLMs. To the best of our knowledge, this is the first practical solution that introduces logical reasoning with LLMs for user preferences to the recommendation domain.
    \item REKA transforms the open-world knowledge to dense vectors in recommendation space, which are compatible with any recommendation models. We also release the code of REKA and the generated textual knowledge from LLMs\footnote{Code and knowledge are available at \url{https://github.com/YunjiaXi/Open-World-Knowledge-Augmented-Recommendation}} to facilitate future research.
    \item We devise collective knowledge extraction for large-scale scenarios to achieve resource efficiency. The knowledge augmentation can be preprocessed and prestored for fast training and inference, avoiding the large inference latency when adopting LLMs to RSs. Now, REKA has been deployed to Huawei's news and music recommendation platforms and gained a 7\% and 1.99\% improvement in the online A/B test. This is one of the first successful attempts in deploying LLM-based recommender to real-world applications.
\end{itemize}
Extensive experiments conducted on public datasets also show that REKA significantly outperforms the state-of-the-art models, and is compatible with various recommendation algorithms. We believe that REKA not only sheds light on a way to inject the knowledge from LLMs into the recommendation models, but also provides a practical framework for open-world recommender systems in large-scale applications.

% we identify major factors that determine user preferences, and break down the compositional preference reasoning problem into simpler subproblems of reasoning each individual factor in our designed \textit{factorization prompting}. The reasoning knowledge on users and the factual knowledge on items are then generated by LLMs with the factorization prompting. 

% Due to the excessive computational cost, LLMs cannot employ real-time user feedback to update and refine the model as in classical recommenders, and hence may fall short in capturing user's recent feedback.
% 3) Another issue that prevents LLMs from practical use is its large inference complexity. With billions of users and thousands of user behaviors in real-world recommendation scenarios, using LLMs directly as recommenders could lead to intractable response times. 

 % LLMs often suffers from \textit{compositional gap} that the model do not generate the correct answer to the compositional question but can correctly answer all its sub-questions. Unfortunately, inferring user's preferences belongs to such compositional problem involving multiple reasoning steps and composing multiple facets of user interest. Thus, LLMs may not be bale to directly do preference reasoning accurately and previous work~\cite{liu2023chatgpt,chatrec,hou2023large} that expects LLMs to directly provide precise answer to the user preference might be overly ambitious. 
 
% Classical recommenders often employ real-time user feedback to update and refine the model, which is currently beyond the capability of LLMs due to excessive computational cost. \xx{unsuitable reasoning approaches} 

% . Possible reasons could include that,, which are mostly numerical and in tabular form
% For example, Liu \textit{et al.}~\cite{liu2023chatgpt} construct task-specific prompts and investigate the recommendation performance of ChatGPT. 

% Click-through rate (CTR) prediction is a crucial task in recommender systems, sharing similar input-output characteristics with many recommendation tasks. In this work, we focus on CTR prediction as the basic task of our framework and this section introduce its formulation and the basic structure. However, it is important to note that our framework is extendable to other recommendation tasks as well.

\section{Preliminaries}\label{sect:network_structure}
In this section, we formulate the recommendation task and introduce the notations. The recommendation task is generally formulated as a binary classification problem over multi-field categorical data. The dataset is denoted as $\mathcal D = \{(x_1, y_1), \ldots, (x_i, y_i), \ldots, (x_n, y_n)\}$, where $x_i$ represents the categorical features for the $i$-th instance and $y_i$ denotes the corresponding binary label (0 for no-click and 1 for click). Usually, $x_i$ contains sparse one-hot vectors from multiple fields, such as item ID and genre. We can denote the feature of the $i$-th instance as $x_i=[x_{i,1}, x_{i,2},\ldots,x_{i, F}]$ with $F$ being the number of field and $x_{i, k}$, $k=1,\ldots,F$ being the feature of the corresponding field. 

Recommendation models usually aims to learn a function $f(\cdot)$ with parameters $\theta$ that can accurately predict the click probability $P(y_i=1|x_i)$ for each sample $x_i$, that is $\hat{y_i} = f(x_i;\theta)$. In practice, industrial recommender systems are confronted with massive users and items. Thus, their recommendation is usually divided into multiple stages, \ie, candidate generation, ranking, and reranking~\cite{liu2022neural}, where different models are used to narrow down the relevant items.
 
However, these classical recommendation models are typically trained on a specific recommendation dataset (\ie, a closed system), overlooking the potential benefits of accessing open-world knowledge. 
% In this work, our proposed framework enables the integration of open-world knowledge from LLMs into various recommendation tasks and stages, enhance the efficacy of recommendations.

% Recommendation models are trained to learn a function $f(\cdot)$ with parameters $\theta$ that can accurately predict the click probability $P(y_i=1|x_i)$ for each sample $x_i$, that is $\hat{y_i} = f(x_i;\theta)$. The model is typically trained with Binary Cross-Entropy (BCE) loss:
% \begin{equation}
% \mathcal{L}=-\sum_{i=1}^n y_{i}\log \hat{y}_{i} + (1-y_{i})\log(1-\hat{y}_{i})\,.
% \end{equation}
 
% However, these classical models are typically trained on a specific recommendation dataset (\ie, a closed system), overlooking the potential benefits of accessing open-world knowledge.

% Accurately predicting the probability of a user clicks an item, \ie, the Click-Though Rate (CTR) prediction, is the core task for recommender systems. \Jianghao{Click-though Rate (CTR) prediction is the core task for recommender systems, where we aim to accurately estimating the user click probability towards a target item.}

% CTR prediction can be formulated as a binary classification problem over multi-field categorical data. The dataset is denoted as $\mathcal D = \{(x_1, y_1), \ldots, (x_i, y_i), \ldots, (x_n, y_n)\}$, where $x_i$ represents the categorical features for the $i$-th instance and $y_i$ denotes the corresponding binary label (0 for no-click and 1 for click). Usually, $x_i$ contains sparse one-hot vectors from multiple fields, such as item ID and genre. We can represent the feature as $x_i=[x_{i,1}, x_{i,2},\ldots,x_{i, F}]$ with $F$ being the number of field and $x_{i, k}$, $k=1,\ldots,F$ being the feature of the corresponding field. 

% Earlier work focuses on the feature interactions between different fields such as DCN \cite{DCN}, DeepFM \cite{DeepFM}, FibiNet \cite{FiBiNET}, AutoInt \cite{AutoInt}, which can be formulated as 
% % \begin{equation}
%     \hat{y_i} = f(x_i;\theta)\,,
%      \label{eq:ctr-goal-1}
% \end{equation}
% where $f$ is the learned function with parameters $\theta$. Recent studies emphasize sequential behavior modeling like DIN \cite{DIN} or DIEN~\cite{DIEN} and incorporate the user behavior sequence $h_i$ together with the current sample $x_i$. Hence the task can be extended to
% \begin{equation}
%     \hat{y_i} = f(x_i,h_i;\theta)\,.
%      \label{eq:ctr-goal-2}
% \end{equation}

% % \subsection{Basic Network Structure}\label{sect:network_structure}
% Typically, the CTR models may have the following four layers: (1) \textit{embedding layer}; (2) \textit{feature interaction layer}; (3) \textit{user behavior modeling layer}; and (4) \textit{output layer} \cite{zhang2021deep}. The categorical features are first converted into low-dimensional dense embeddings in the embedding layer. Then the embeddings are fed into the feature interaction layer to capture complex relationships and high-order interactions, enabling the model to learn non-linear patterns. Meanwhile, the user behavior modeling layer models captures user interests and preferences based on historical behavior or contextual information, utilizing techniques like RNNs or attention mechanisms to capture temporal dependencies. Finally, the output layer takes the processed features and generates the final prediction of the click probability, usually using a linear or MLP layer followed by a sigmoid activation function.



 % and other dense features \Jianghao{The continuous features are also fed into the embedding layer (lots of work analyze how to embed continuous features). I suggest omit continuous features here.}



% The categorical features are first converted into low-dimensional dense embeddings in the embedding layer, where $x_{i,j}$ are transformed into $e_{i,j}$ so as to get the embedding $e_i=[e_{i,1};e_{i,2};\ldots;e_{i,F}]\in\mathbb{R}^{F\times d}$ of $i$-th instance with $d$ being the embedding size. Then the feature interaction layer combines embeddings and other continuous features to capture complex relationships and high-order interactions, enabling the model to learn non-linear patterns. Meanwhile, the user behavior modeling layer models user interests and preferences based on historical behavior or contextual information, utilizing techniques like RNNs or attention mechanisms to capture temporal dynamics and long-term dependencies. Finally, the output layer takes the processed features and generates the final prediction of the click probability, usually using a linear or MLP layer followed by a sigmoid activation function. After obtaining the predictions from the output layer, the model is typically trained with Binary Cross-Entropy (BCE) loss:

% Note that not all models include all four components mentioned above. Depending on whether the model emphasizes sequence modeling or feature interactions, it may have either the feature interaction layer or the interest modeling layer.

% \textbf{Embedding layer} is responsible for transforming categorical features into low-dimensional dense embeddings, that is to transform $x_{i,j}$ into $e_{i,j}$ so as to get the embedding $e_i=[e_{i,1};e_{i,2};\ldots;e_{i,F}]\in\mathbb{R}^{F\times d}$ of $i$-th instance with $d$ being the embedding size.


% \textbf{Feature interaction layer} combines the embeddings and possibly other continuous features to capture complex relationships and high-order interactions between different features. It applies operations like inner/outer product, neural network, and attention, allowing the model to capture non-linear patterns and interactions within the data.

% \textbf{User behavior modeling layer} focuses on modeling the user's interests and preferences based on historical behavior or contextual information. It can incorporate techniques like recurrent neural networks (RNNs) or attention mechanisms to capture temporal dynamics and long-term dependencies in the user's sequential behavior, providing a accurate representation of user interests.


% \textbf{Output layer} takes the processed features from the previous layers and produces the final prediction or click probability. It typically involves a single linear or MLP layer followed by a sigmoid activation function, representing the estimated probability of a user clicking on a specific item or advertisement. 


\section{Methodology}
We first provide an overview of our proposed Open-World Recommendation Framework with Efficient Knowledge Augmented from Large
Language Models, and then elaborate on the details of each component.

\subsection{Overview}
To extract open-world knowledge from LLMs and incorporate it into RSs, we design REKA, as shown in Figure~\ref{fig:open_world}. This framework is model-agnostic and consists of the following three stages: 

\smallskip
\noindent
\textbf{Knowledge Reasoning and Generation Stage} leverages our designed factorization prompting to extract recommendation-relevant knowledge from LLMs. We first decompose the complex reasoning tasks by identifying major scenario-specific factors that determine user preferences and item characteristics. Then, according to different scales of recommendation scenarios, we devise two knowledge generation approaches with those factors. The individual knowledge extraction for the small scenarios  utilizes LLMs to generate individual knowledge about the scenario-specific factors for each item and user. In collective knowledge extraction for large scenarios, we first cluster the user and item into groups, respectively, and then require LLMs to generate knowledge for each group according to scenario-specific factors. Thus, we can obtain open-world knowledge about the user and item beyond the original recommendation dataset. 

% \Jianghao{This part is quite confusing. I suggest using `itemize` to introduce the two different prompts.}
% The direct knowledge on items and indirect knowledge on user preferences are then generated by LLMs with item and preference prompts, respectively. 

\smallskip
\noindent
\textbf{Knowledge Adaptation Stage} converts textual open-world knowledge into compact and relevant representations suitable for recommendation, bridging the gap between LLMs and RSs. First, the user and item knowledge obtained from LLMs are encoded into dense representations by a knowledge encoder. Next, a hybrid-expert adaptor is designed to transform the representations from the semantic space\footnote{the embedding space from language models} to the recommendation space. In this way, we obtain the user augmented vector for user preferences and the item augmented vector for each candidate item.  

% \Jianghao{natural language space? Since we also mention `semantic` in literal CTR prediction papers}

\smallskip
\noindent
\textbf{Knowledge Utilization Stage} integrates the user and item augmented vectors into an existing recommendation model, enabling it to leverage both domain knowledge and open-world knowledge during the recommendation process. 

The knowledge generation and encoding are conducted through preprocessing. The hybrid-expert adaptor and recommendation model are jointly trained in an end-to-end manner.




\subsection{Knowledge Reasoning and Generation}
As the model size scales up, LLMs can encode a vast array of world knowledge and have shown emergent behaviors such as the reasoning ability~\cite{qiao2023reasoning,huang2022reasoning}. This opens up new possibilities for incorporating user-side knowledge of user preferences and factual knowledge for candidate items in recommendation systems. However, it is non-trivial to extract those two kinds of knowledge from LLMs due to the following three challenges.

Considering the user-side knowledge that requires the reasoning ability of LLMs, according to~\cite{press2022measuring}, LLMs often suffer from the \textit{compositional gap} where the model fails at generating the correct answer to the compositional question but can correctly answer all its sub-questions. Users' clicks on items are motivated by multiple key aspects and users' interests are diverse, and multifaceted, which involve multiple reasoning steps. To this end, LLMs may not be able to produce accurate reasoning knowledge directly. Expecting LLMs to provide precise recommendations in one step as in previous work~\cite{liu2023chatgpt,chatrec,hou2023large} might be overly ambitious. 
% By breaking down the complex preference reasoning problem into simpler subproblems of reasoning according to each individual factor, the compositional problem can be alleviated and correlations of different factors behind the user preferences can be analyzed.

As for factual knowledge about items, LLMs contain massive world knowledge, yet not all of it is useful for recommendation. When the request to an LLM is too general, the generated factual knowledge may be correct but useless, as it may not align with the inferred user preferences. For example, an LLM may infer that a user may prefer highly acclaimed movies that have received multiple awards, while the generated factual knowledge is about the storyline of the target movie. This mismatch between user-side knowledge and item factual knowledge may limit the performance of RSs. 

More importantly, the majority of recommendation systems in the industry may face the challenge of dealing with billions of users and items. Given the enormous parameter size of LLMs, the time and resources for generating knowledge can be considerable. Taking into account the frequent model updates required by industrial recommendation systems and resource constraints, generating knowledge for each user and item becomes impractical in large-scale recommendation scenarios.

% As for the factual knowledge, LLMs contain massive world knowledge, yet not all of them are useful for recommendation. By augmenting the items with the preference-sensitive feature factors, the recommender systems can easily match the attracting items to the users. For example, the LLM infers that a user may prefer highly acclaimed movies that have received multiple awards, based on the user's history and the external knowledge it possesses. However, in a movie recommendation dataset, the awards of the movies may not be available. Incorporating the award knowledge from the LLMs can help align the items to the user preferences, enables more accurate and personalized recommendations. 

Therefore, inspired by the success of Factorization Machines \cite{rendle2010factorization} in RSs, we design \textit{factorization prompting} to explicitly "factorize" user preferences and item knowledge into several major factors for effectively extracting the open-world knowledge from LLMs. Then, with the factors incorporated into the prompt design, the complex reasoning and knowledge extraction problem can be broken down into simpler subproblems for each factor, thus alleviating the compositional gap of LLMs. In addition, we devise distinct knowledge generation approaches for recommendation scenarios of different scales. For relatively smaller scenarios, we implement individual knowledge extraction, where the item prompt and user prompt are designed for each user and item, facilitating the generation of individual knowledge. In contrast, we introduce collective knowledge extraction for larger scenarios with a considerable number of users and items, which involves clustering users and items first and then prompting collective knowledge for each cluster.

% Besides, we also design \textit{item prompt}, which utilizes those factors to extract factual knowledge relevant to user preferences. This ensures the generated reasoning knowledge and factual knowledge are aligned for the effective utilization in RSs.



\begin{figure*}
    \centering
    % \vspace{-4pt}
    \includegraphics[width=\textwidth]{imgs/LLM4RS-prompt-group.pdf}
    % \vspace{-3pt}
    \caption{Example prompts for REKA. The green, purple, and yellow text bubbles represent the prompt template, the content to be filled in the template, and the real response generated by LLMs, respectively (some text has been omitted due to the page limits).}
    % \vspace{-3pt}
    \label{fig:promp}
\end{figure*}

% \xx{It's not straightforward to reason on user preference and generate item factual knowledge that is useful for RSs. ...two challenges:compositional gap, massive item knowledge....our solution:factorization prompting...}

% Therefore, we propose to explicitly decompose user preference and item characteristics into different factors, which further prompts LLMs to reason user preferences and provide related item factual knowledge, motivated by~\cite{press2022measuring, zhou2023leasttomost}, 

% Therefore, we 
% Reasoning is a fundamental aspect of human intelligence and provides back-end support for various real-world applications \Jianghao{Weird that reasoning provides back-end support for various real-world applications}. In the field of recommendation, the reasoning ability is also crucial since it allows the system to go beyond learning the simple correlations and uncover underlying patterns and connections among user behaviors. It helps us understand the \textit{"why"} behind user preferences, and enables more accurate and personalized recommendations. However, traditional recommendation models primarily focus on leveraging statistical techniques and collaborative signals because it is difficult for these light-weight neural networks to reason from the input data. Fortunately, In this work, to better elicit the reasoning ability of LLMs for extracting open-world knowledge related to recommendation, we design \textit{factorization prompting} by first factorizing user preferences and then utilizing the obtained factors for prompting.

% Though excelling at capturing underlying correlations and patterns, LLMs may struggle to directly solve complex tasks that consist of multiple reasoning steps. According to~\cite{press2022measuring}, LLMs often suffer from the \textit{compositional gap} where the model fails at generating the correct answer to the compositional question but can correctly answer all its sub-questions. User's clicks on items is motivated  by multiple key aspects and users' interests are diverse and multifaceted, which involve multiple reasoning steps. To this end, LLMs may not be able to directly produce accurate preference reasoning results. Expecting LLMs to provide precise recommendation in one step as in previous work~\cite{liu2023chatgpt,chatrec,hou2023large} might be overly ambitious. Moreover, even if the LLMs can accurately infer user preferences, the lack of corresponding knowledge of item in dataset may hinders the effective utilization of preference by the RSs. For example, the LLM infers that a user may prefer highly acclaimed movies that have received multiple awards, based on the user's history and the external knowledge it possesses. However, in a movie recommendation dataset, the awards of the movies may not be available. Even when relying on LLMs to provide item-related knowledge, the knowledge can be too chaotic to align with  the exact user preference information. As a result, the RS may fail to match the corresponding movies to the user. Therefore, elaborate design of prompt strategy for inferring user preference and extracting related item factual knowledge is necessary to align the obtained knowledge more effectively.

% \vspace{-3pt}
\subsubsection{Scenario-specific Factors} 

% \Jianghao{... solve complex reasoning tasks that could be reduced to a chain of thought steps}
% Therefore, it is necessary to augment the candidate items with factual knowledge aligned with user preferences, such as their awards information.
 % User preferences are inherently complicated and multifaceted,

The factors determining user preferences may vary for different recommendation scenarios. To determine the factors for different scenarios, we rely on a combination of interactive collaboration with LLMs and expert opinions. For example, in movie recommendation, given a prompt "\textit{List the important factors or features that determine whether a user will be interested in a movie}", LLMs can provide some potential factors. Then, we involve human experts to confirm and refine the outputs to acquire the final scenario-specific factors for movie recommendation --- including \textit{genre, actors, directors, theme, mood, production quality, and critical acclaim}. Similarly, in news recommendation, we may obtain factors like \textit{topic, source, region, style, freshness, clarity, and impact}. The collaborative process between LLMs and experts ensures that our chosen factors encompass the critical dimensions of user preference and item characteristics for each scenario. 

Note that the specification of these factors is required only once for each scenario and it does not demand much domain expertise with the aid of LLMs. This shows that the proposed method can be easily generalized to different scenarios with little human intervention and manual effort.

% \xx{While there is human intervention involved here, it is required only once for each scenario. Compared to the extensive human annotation required for knowledge graph, the human involvement in this case is minimal and relatively straightforward.}

% The scenario-specific factors will be leveraged in following prompt designed for user preference reasoning and item factual knowledge generation. On one hand, incorporating scenario-specific factors into the preference reasoning prompt can alleviate the compositional gap. LLMs only need infer user preferences regarding to those factors separately, making preference reasoning task more manageable for LLMs. On the other hand, including the same factors in the prompt for item factual knowledge generation enable LLMs to generate aligned knowledge that is relevant to user preference. This ensure the generated knowledge can be effectively utilized by the RSs


% This not only allows LLMs to solve the preference reasoning problem more easily with less compositional gap and 
% By breaking down user preference, we allow LLMs to recall more
% detailed knowledge and solve the preference reasoning problem
% more easily, thereby alleviating the compositional gap problem and fully leveraging the reasoning capabilities of LLMs

% \Jianghao{This section only talks about preference reasoning prompt?}
 

% Such complex reasoning ability is usually unlocked by specific prompting strategies, e.g., generated knowledge prompting~\cite{}, and problem decomposition ~\cite{}. 

\subsubsection{Individual Knowledge Extraction} After obtaining the scenario-specific factors, we introduce them into our first prompt engineering approach -- individual knowledge extraction. This approach is designed explicitly  for smaller scenarios where the number of users and items is not substantial. In such scenarios, it is feasible to employ LLMs to generate individual knowledge for each user and item. Specifically, we propose to apply the LLM as a preference reasoner to infer user preferences, and a knowledge provider to acquire external factual knowledge for candidate items. Therefore, we design two types of prompts accordingly: user prompt and item prompt, as illustrated in Figure~\ref{fig:promp}(a) and Figure~\ref{fig:promp}(b).


\textbf{User prompt} is constructed with the user's profile description, behavior history, and scenario-specific factors. Figure~\ref{fig:promp}(a) shows an example of the prompt and real response from the LLM, where the user profile description and behavior history provide the LLM with the necessary context and user-specific information to understand the user's preferences. Scenario-specific factors can instruct the LLM to analyze user preference from different facets and allow the LLM to recall the relevant knowledge more effectively and comprehensively. For example, in the factor of genre, the LLM infers user preference for genres such as thriller, comedy, and animation based on user's positive ratings on thriller movies like \textit{What Lies Beneath}, \textit{Scream}, as well as comedy animations like \textit{Toy Story} and \textit{Aladdin}. With the designed prompt, LLM can successfully analyze the user's preferences toward corresponding factors, which is beneficial for recommendations.
 % We can observe that in the generated response, the LLM analyzes and identifies the user's preferences for the corresponding factors based on the user's profile and behavior history, which is beneficial for recommendations.

% Instructing the LLM to analyze the user preference according to the scenario-specific factors allows the LLM to recall the relevant knowledge more effectively and comprehensively.

\textbf{Item prompt} is designed to fill the knowledge gap between the candidate items and the generated user-side knowledge. Since the dataset in RS may lack relevant knowledge about scenario-specific factors from items, we need to extract corresponding knowledge from LLM to align the generated user and item knowledge.  As illustrated in Figure~\ref{fig:promp}(b), an item prompt consists of two parts -- the target item description and the scenario-specific factors. This prompt can guide LLM in compensating for the missing knowledge within the dataset. For instance, in Figure~\ref{fig:promp}(b), LLM supplements \textit{Roman Holiday} with \textit{"a light and playful tone"}, which is rarely recorded in the datasets. In this way, LLM provides external knowledge that aligns with user preferences, allowing for more accurate and personalized recommendations.

 By combining the two kinds of prompts, we enable the LLM to act as both a preference reasoner and a knowledge provider, thereby extracting individual user and item knowledge from LLMs. We refer to the generated textual response with the user and item prompt as the \textit{user knowledge} and the \textit{item knowledge}, respectively.

\subsubsection{Collective Knowledge Extraction} In the preceding section, the individual knowledge extraction that we devised proves effective in scenarios characterized by a relatively limited number of users and items. In this approach, we employ prompts to extract knowledge for each user and item. However, owing to the substantial time and resource consumption involved in generating knowledge through LLMs, the feasibility of extracting knowledge for each user and item becomes questionable when we confront larger recommendation scenarios housing a significant number of users and items. Consequently, for larger recommendation scenarios, we have introduced collective knowledge extraction. This approach first conducts user and item clustering, with each cluster represented by a set of items. Subsequently, we have formulated a unified prompt designed for both user and item to extract knowledge for each cluster in Figure~\ref{fig:promp}(c). Regulating cluster size through clustering algorithms affords us the flexibility to manage the number of clusters, thereby controlling the time and resource consumption during the knowledge generation.

Conventional clustering methods, such as k-means and standard hierarchical clustering, often face challenges in handling data within large-scale recommendation scenarios. Firstly, they exhibit high complexity when dealing with large-scale and high-dimension data. Secondly, they lack scalability, struggling to accommodate the continuous arrival of new users or items in dynamic recommendation scenarios. To address these limitations, we choose a streaming hierarchical clustering approach, StreaKHC~\cite{xing2022streaming} algorithm to cluster users and items. Leveraging a scalable point-set kernel, StreaKHC is capable of handling large volumes of streaming data in recommendation scenarios. It employs a top-down search strategy to recursively add a new point to the most similar child node, resulting in a time complexity of $O(n)$. Additionally, as a hierarchical clustering algorithm, it forms a tree structure, allowing us to change the number of clusters without regenerating the entire tree.

\textbf{Item clustering} is a relatively straightforward process. Initially, we pre-train embeddings for all items using traditional recommendation models such as DIN~\cite{DIN}. Subsequently, these item embeddings are then fed into the StreaHKC algorithm for clustering, resulting in multiple clusters. Each item cluster, denoted as $c^a_i$, comprises multiple items represented as $c^a_i=\{a_1,\ldots, a_k,\ldots,a_m\}$, where 
$a_k$ represents an item, and 
$m$ denotes the number of items within that cluster. The maximum value of $m$ can be controlled indirectly through parameters in the StreaHKC algorithm, so we can regulate the number of clusters. The StreaHKC algorithm forms a tree structure. Hence, when some new items arrive, we can efficiently introduce new nodes into this tree and swiftly obtain new clusters through a splitting algorithm.

\textbf{User clustering} becomes more intricate due to the nature of user representation in recommendation systems, where users are typically identified by IDs without corresponding textual descriptions, unlike items.  Consequently, it is challenging for unfine-tuned \ww{untuned} LLMs to comprehend user representations in this format. Thus, we adopt a strategy where a user is represented by a set of \ww{commonly-interested} items, specifically the items the user has recently clicked. Correspondingly, when clustering users, each cluster should also be a set of items, enabling LLMs to comprehend the cluster for knowledge reasoning and extraction.

To implement this, we leverage the same item embeddings pre-trained mentioned in the item clustering phase. For a user 
$u_k$, the average of embeddings for all items recently clicked by the user serves as the user representation. After inputting all user representations into the StreaKHC algorithm, we obtain each user cluster, $c^u_i=\{u_1,\ldots,u_k,\ldots,u_t\}$, where $u_k$ represents a user and $t$ is the number of users in that cluster. At this point, the user cluster we obtain is still represented by a set of users, which needs to be transformed into a set of items for LLMs' comprehension. To achieve this, we extract common historical items from all users within each cluster $c^u_i$, forming a new representation for the user cluster, i.e., $\hat{c}^u_i=\{a_1,\ldots,a_k,\ldots,a_s\}$, where 
$s$ is the total number of items in the cluster, and $a_k$
  represents items appearing in the click history of at least $d$ users within $c^u_i$. Here, $d$ denotes a hyper-parameter that can be set.
\ww{$\hat{c}^u_i$ is not very clearly described.}

\textbf{User/item prompt} in collective knowledge extraction is designed for extracting the commonalities within a set of items, \ie, collective knowledge. This is because each cluster obtained from the previous user and item clustering stage is represented by a set of items. Consequently, we have crafted identical prompts for user and item clusters, as depicted in Figure~\ref{fig:promp}(c), which comprises set description and scenario-specific factors. Here, the set description refers to each cluster obtained from user and item clustering, represented by a set of items. Similar to prompts in individual knowledge extraction, the item and user prompts require scenario-specific factors to guide LLMs in analyzing the shared characteristics of this set of items. For instance, in Figure~\ref{fig:promp}(c), regarding themes, the LLM can infer that this set of movies \ww{``}explores complex and often contradictory aspects of human relationships\ww{"}. In terms of characters, \ww{``}these movies often feature complex characters\ww{"}. Through this prompt, LLMs can effectively reason and extract the commonalities within a set of items, \ie, their collective knowledge.

% \vspace{-5pt}
\subsection{Knowledge Adaptation}
The knowledge generated by LLMs presents new challenges in harnessing its potential to assist recommendation models: 1) The knowledge generated by LLMs is usually in the form of text, which cannot be directly leveraged by traditional RSs that typically process categorical features. 2) Even if some LLMs are open-sourced, the decoded outputs are usually large dense vectors (\eg, 4096 for each token) and lie in a semantic space that differs significantly from the recommendation space. 3) The generated knowledge may contain noise or unreliable information~\cite{ji2023survey}. 

To address these challenges, we have devised two modules: a \textit{knowledge encoder} and a \textit{hybrid-expert adaptor}. The knowledge encoder module encodes the generated textual knowledge into dense vectors and aggregates them effectively. The hybrid-expert adaptor converts dense vectors from the semantic space to the recommendation space. It tackles dimensionality mismatching and allows for noise mitigation. Thus, the knowledge adaptation stage increases the reliability and availability of  generated knowledge and bridges gap between LLMs and RSs.

\subsubsection{Knowledge Encoder} To harness the potential of textual knowledge generated by LLMs, we employ a knowledge encoder, \eg, BERT~\cite{bert}, to obtain the encodings for each token within the text. Then, we require an aggregation process that combines each token to generate the \textit{user representation} $r^u_i\in\mathbb{R}^{m}$ and the \textit{item  representation} $r^\iota_i\in\mathbb{R}^{m}$ of size $m$ as follows
\begin{equation}
    \begin{split}       
    &r^p_i = \text{Aggr}(\text{Encoder}(klg^u_i))\,, \\
    &r^\iota_i = \text{Aggr}(\text{Encoder}(klg^\iota_i))\,,
    \end{split}
\label{eq:aggr_encoder}
\end{equation}
where $klg^u_i$ and $klg^\iota_i$ denote the user knowledge and item knowledge generated by LLMs of the $i$-th instance in the dataset. Here, various aggregation functions can be employed, such as the representation of the [CLS] token and average pooling. In practice, we primarily adopt average pooling. Note that the knowledge encoder is devised for situations where we only have access to the textual outputs of LLMs. The separate knowledge encoder can be eliminated if the dense vector outputs from LLMs are available.
% In practice, we primarily adopt average pooling, but we also explore the effectiveness of other aggregation methods.

% the representation of the last token \Jianghao{Suggest remove `the representation of the last token`; cls and average pooling are OK.},

\subsubsection{Hybrid-expert Adaptor} To effectively transform and compact the attained aggregated representations from the semantic space to the recommendation space, we propose a hybrid-expert adaptor module. The aggregated representations capture diverse knowledge from multiple aspects, so we employ a structure that mixes shared and dedicated experts, inspired by the Mixture of Experts (MoE)~\cite{MoE} approach. This allows us to fuse knowledge from different facets and benefit from the inherent robustness offered by multiple experts. 
% \cb{why not use OpenRec directly?}

In particular, to fully exploit the shared information of the user representation and the item representation, we have designed both shared experts and dedicated experts for each kind of representation. 
The shared experts capture the common aspects, such as shared features, patterns, or concepts, that are relevant to both user and item knowledge. User and item representations also have their dedicated sets of experts to capture the unique characteristics specific to the user or item knowledge. 
Mathematically, denote $\mathcal S_s$, $\mathcal S_u$, and $\mathcal S_\iota$ as the sets of shared experts and dedicated experts for user and item knowledge with the expert number of $n_s$, $n_u$ and $n_\iota$. The output is the \textit{user augmented vector} $\hat{r}_{i}^u\in\mathbb{R}^{q}$ and the \textit{item augmented vector} $\hat{r}_{i}^\iota\in\mathbb{R}^{q}$ of size $q$ ($q$ is much less than the original dimension $m$), which are calculated as follows
\begin{equation}
\begin{split}
    \alpha^u_{i} &=\operatorname{Softmax}(g^u(r^u_i))\,,\quad\alpha_{i}^\iota =\operatorname{Softmax}(g^\iota(r^\iota_i))\,,\\
    \hat{r}_{i}^u&=\sum\nolimits_{e\in \mathcal S_s} \alpha_{i,e}^u \times e(r^u_i) + \sum\nolimits_{e\in \mathcal S_u} \alpha_{i,e}^u \times e(r^u_i)\,,\\
    \hat{r}_{i}^\iota&=\sum\nolimits_{e\in \mathcal S_s} \alpha_{i,e}^\iota \times e(r^\iota_i) + \sum\nolimits_{e\in \mathcal S_\iota} \alpha_{i,e}^\iota \times e(r^\iota_i)\,,\\
\end{split}
\end{equation}
where $g^u(\cdot)$ and $g^\iota(\cdot)$ are the gating networks for user and item representations, and their outputs $\alpha^u_i$ and $\alpha^\iota_i$ are of size $n_s+n_u$ and $n_s+n_\iota$. Here $e(\cdot)$ denotes the expert network, and $\alpha_{i,e}^u$ and $\alpha_{i,e}^\iota$ are the weights of expert $e(\cdot)$ generated by the gating network for user and item, respectively. Here, each expert network $e(\cdot)$ is designed as a Multi-Layer Perceptron (MLP), facilitating dimensionality reduction and space transformation. Empirical experiments show that about 5 experts are sufficient to generate a satisfying performance\footnote{There is no need to set a large number of experts here, and thus, the model does not suffer from convergence issues.}.
% \xx{Empirical experiments show that there is no need to set a large number of experts here, and thus, the model does not suffer from convergence issues.}
% \cb{the optimization of this stage is missing}

\subsection{Knowledge Utilization}
Once we have obtained the user augmented vector and the item augmented vector, we can then incorporate them into backbone recommendation models. This section explores a straightforward approach where these augmented vectors are directly treated as \textbf{additional input features}. Specifically, we use them as additional feature fields in recommendation models, allowing them to interact with other features explicitly. During training, the hybrid-expert adaptor module is jointly optimized with the backbone model to ensure the transformation process adapts to the current data distribution. Generally, REKA can be formulated as
\begin{equation}
    \hat{y_i} = f(x_i,h_i,\hat{r}_{i}^u,\hat{r}_{i}^\iota;\theta)\,,
     \label{eq:ctr-goal-3}
\end{equation}
which is enhanced by the the user augmented vector $\hat{r}_{i}^u$ and the item augmented vector $\hat{r}_{i}^\iota$. Importantly, REKA only modifies the input of the backbone model and is independent of the design and loss function of the backbone model, so it is flexible and compatible with various backbone model designs. Furthermore, it can be extended to various recommendation tasks, such as sequential recommendation and direct recommendation, by simply adding two augmented vectors in the input. By incorporating the knowledge augmented vectors, REKA combines both the open-world knowledge and the recommendation domain knowledge in a unified manner to provide more informed and personalized recommendations.

% Importantly, our proposed REKA can be applied for different backbone models and loss functions, demonstrating its flexibility and compatibility.

% \vspace{-6pt}
\subsection{Speed-up Approaches for Knowledge Utilization}\label{sec:speed_up}
Our proposed REKA framework adopts LLMs to generate knowledge for user preferences and candidate items. Due to the immense scale of the model parameters, the inference of LLMs takes extensive computation time and resources, and the inference time may not meet the latency requirement in real-world recommender systems with large user and item sets. 

To address this, we employ an acceleration strategy to \textbf{prestore knowledge representations} $r^u_i$ and $r^\iota_i$ generated by the knowledge encoder or the LLM into a database. As such, we only use the LLM and knowledge encoder once before training backbone models. During the training and inference of the backbone model, relevant representations are retrieved from the database. Besides, the efficiency of offline knowledge generation with LLM can further be enhanced via quantization or hardware acceleration techniques.
% \Jianghao{Suggest: During the training and inference stages, according to the user ID and target item ID, knowledge representations are retrieved from the database for the backbone model.} 
% \Jianghao{Suggest new paragraph here. Next is other further speedup for inference.}
% \Jianghao{$r^p_i$ and $r^\iota_i$ are generated by knowledge encoder, instead of LLM. Suggest: prestore the knowledge representation $r^p_i$ and $r^\iota_i$ generated by the knowledge encoder in the adaptation stage into a database}

If we have stricter requirements for inference time or storage efficiency, we can detach the adaptor from the model after training and further \textbf{prestore augmented vectors} \ie, $\hat{r}_{i}^u$ and $\hat{r}_{i}^\iota$, for inference. The dimension of the augmented vectors (\eg, 32) is usually much smaller than that of the knowledge representations (\eg, 4096), which improves the storage efficiency. Additionally, prestoring the augmented vectors reduces the inference time to nearly the same as the original backbone model, and we have provided experimental verification in Section~\ref{sec:speed_up_efficiency}. In particular, assume the inference time complexity of the backbone model is $O(f(n, m))$, where $n$ is the number of fields and $m$ is the embedding size. The polynomial function $f(n,m)$ varies depending on different backbone models. With REKA, the inference time complexity is $O(f(n+2,m))=O(f(n,m))$, which is equivalent to the complexity of the original model. 

% In particular, assume the inference time complexity of backbone model is $O(f(n))$, where $n$ is the number of fields and $f(n)$ varies depending on different backbone models. In our framework, the inference time complexity is $O(f(n+2))=O(f(n))$, which is equivalent to the complexity of original model. 
% \Jianghao{Complexity should be $O(f(n,m))$, where $n$ is the number of fields and $m$ is the embedding size.}
% \Jianghao{$f(n,m)$ is a polynomial function, which varies depending on different backbone models}

Since item features are relatively fixed and do not change frequently, it is natural and feasible to prestore the item knowledge for further use. Moreover, user behaviors evolve over time, making it challenging for LLMs to provide real-time user-side knowledge about behaviors. However, considering that long-term user preferences are relatively stable, and the backbone model already emphasizes modeling recent user behaviors, it is unnecessary to require LLMs to have access to real-time behaviors. Therefore, LLM can infer long-term preferences based on users' long-term behaviors, allowing for conveniently prestoring the generated knowledge without frequent updates. As such, the inference overhead of LLMs can also be significantly reduced. The backbone models can capture ever-changing short-term preferences with timely model updates.  This can take better advantage of both LLMs and recommendation models. Similar to common practice for cold start users or items~\cite{zhang2014addressing}, we use default vectors when encountering new users or items at inference time. Subsequently, we will generate the knowledge for those new users and items offline and add them to the database.

% Therefore, LLM can infer long-term preferences based on users' long-term behaviors, allowing for convenient prestore generated knowledge without frequent updates. Moreover, encouraging LLMs to focus on long-term preferences while the backbone model to attend to short-term preferences in real-time feedback which can be updated timely. This can take better advantage of both LLMs and the recommendation models. \cb{we can deconstruct the user preferences into long-term and short-term, for high-activity users, short-term preferences can be updated periodically.}

% In addition, this approach also strikes a balance between modeling long-term and short-term user interests, facilitating more accurate and timely recommendations.

% Prestoring LLM-generated knowledge representations allows for efficient retrieval during the recommendation training and inference, enabling the recommendation model to access to relevant knowledge without relying on real-time LLMs computations. The inclusion of the prestored knowledge representations only introduce two additional feature fields which does not increase the time complexity of backbone model. To be more specific, let us assume 

% Overall, REKA aims to effectively and efficiently allow the classical recommender systems to utilize the open-world knowledge and the reasoning ability of LLMs. The knowledge reasoning and generation stage, as well as the knowledge encoding step, can be preprocessed and prestored to avoid the large computational cost of LLMs during the inference of recommender system. The hybrid-expert adaptor module is jointly trained with the backbone recommendation model. 

% store and retrieval, cutting
% \subsubsection{Time Complexity} 
% almost the same
% generate a response complexity: m
% ctr inference 



==> exp-backup.tex <==
\vspace{-5pt}
\section{Experiment}
% Click-through rate (CTR) prediction is a crucial task in recommender systems, sharing similar input-output formualtion with many recommendation tasks. Thus, this section focuses on evaluating the effectiveness of our proposed framework, REKA, with CTR prediction as the fundamental task. Importantly, REKA is easily extendable to other recommendation tasks. 
To gain more insights into REKA, we tend to address the following research questions (RQs) in this section. 
\begin{itemize}
    \item \textbf{RQ1:} What improvements can REKA bring to backbone models on different tasks, such as CTR prediction and reranking? 
    \item \textbf{RQ2:} How does REKA perform compared with other PLM-based baseline methods?
    \item \textbf{RQ3:} Does the knowledge from LLM outperform other methods of knowledge, such as knowledge graph?
    \item \textbf{RQ4:}Does REKA gain performance improvement when deployed online?
    \item \textbf{RQ5:} Does the acceleration strategy, grouping, preprocessing, and prestorage, enhance the inference speed?
    \item \textbf{RQ6:} How do the reasoning knowledge and factual knowledge generated by the LLM contribute to performance improvement?
    \item \textbf{RQ7:} How do different knowledge adaptation approaches impact the performance of REKA?
    
\end{itemize}
By answering these questions, we aim to comprehensively evaluate the performance and versatility of our proposed framework.
% What roles do the preference and item knowledge generated by the LLM play?
\vspace{-4pt}
\subsection{Setup}
% \footnote{Considering the large API cost of the LLMs, we only conduct experiments on one public dataset.}
\subsubsection{Dataset}
Our experiments are conducted on public datasets, MovieLens-1M\footnote{\url{https://grouplens.org/datasets/movielens/1m/}} and Amazon\footnote{\url{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon_v2/}}. \textbf{MovieLens-1M} contains 1 million ratings provided by 6000 users for 4000 movies. Following the data processing similar to DIN~\cite{DIN}, we convert the ratings into binary labels by labeling ratings of 4 and 5 as positive and the rest as negative. The data is split into training and testing sets based on user IDs, with 90\% assigned to the training set and 10\% to the testing set. The dataset contains user features like age, gender, occupation, and item features like item ID and category. The inputs to the models are user features, user behavior history (the sequence of viewed movies with their ID, category, and corresponding ratings), and target item features. \textbf{Amazon-Book}~\cite{ni2019justifying} is the “Books” category of the Amazon Review Dataset. After filtering out the less-interacted users and items, we remain 11, 906 users and 17, 332 items with 1, 406, 582 interactions. The preprocessing is similar to MovieLens-1M, with the difference being the absence of user features. Additionally, ratings of 5 are regarded as positive and the rest as negative.



% with 51, 311, 621 reviews and 2, 935, 525 books. Due to the large amount of data, we filter out users with fewer than 60 interactions and items with fewer than 40 interactions.

% covering multiple categories. Here we mainly focus on category \textbf{Books}
% \footnote{To avoid the large API cost, we select one of the most commonly used dataset for recommender systems.}
% The features include the ID and category of the target movie, profile features of the user, as well as the ID, category, and rating of the movies that the user has previously viewed. Our goal is to predict whether a user will rate a given movie above 3 (positive label) based on features of the movie and user's historical behaviors. 
% \ljh{backbone model is also a kind of baseline, and the current baseline and comparison are sort of messy. I suggest following baseline classification: (1) ID-based backbone (or baseline), (2) PLM-based baseline, (3) KG-based baseline}
\subsubsection{Backbone Models} Because REKA is a model-agnostic framework, various tasks and models in traditional ID-based recommendation can serve as the backbone model, taking as input the knowledge-augmented vectors generated by REKA. Here, we select two crucial recommendation tasks: \textbf{CTR prediction} and \textbf{reranking}, to validate the effectiveness of REKA across various tasks. CTR prediction aims to anticipate how likely a user is to click on an item, usually used in the ranking stage of recommendation. Reranking is to reorder the items from the previous ranking stage and derive a list that yields more utility and user satisfaction~\cite{liu2022neural}.

We choose 9 representative CTR models as our backbone models, which can be categorized into  user behavior models and feature interaction models. \textbf{User Behavior Models} emphasize modeling sequential dependencies of user behaviors. \textbf{DIN}~\cite{DIN} utilizes attention to model user interests dynamically with respect to a certain item. \textbf{DIEN}~\cite{DIEN} extends DIN by introducing an interest evolving mechanism to capture the dynamic evolution of user interests over time. 

% The former focuses on modeling feature interactions between different feature fields and we adopt widely-used \textbf{DeepFM}~\cite{DeepFM}, \textbf{xDeepFM} \cite{xDeepFM}, \textbf{DCN}~\cite{DCN}, \textbf{DCNv2}~\cite{DCNv2}, \textbf{FiBiNet}~\cite{FiBiNET}, \textbf{FiGNN}~\cite{Fi-GNN}, and \textbf{AutoInt}~\cite{AutoInt}. The latter emphasizes on modeling sequential dependencies of user behaviors and we employ \textbf{DIN}~\cite{DIN} and \textbf{DIEN}~\cite{DIEN}. 

\textbf{Feature Interaction Models} focus on modeling feature interactions between different feature fields. \textbf{DeepFM}~\cite{DeepFM} is a classic CTR model that combines factorization machine (FM) and neural network to capture low-order and high-order feature interactions. \textbf{xDeepFM} \cite{xDeepFM} leverages the power of both deep network and Compressed Interaction Network to generate feature interactions at the vector-wise level. \textbf{DCN}~\cite{DCN} incorporates cross-network architecture and the DNN model to learn the bounded-degree feature interactions. \textbf{DCNv2}~\cite{DCNv2} is an improved framework of DCN which is more practical in large-scale industrial settings. \textbf{FiBiNet}~\cite{FiBiNET} can dynamically learn the feature importance by Squeeze-Excitation network and fine-grained feature interactions by bilinear function. \textbf{FiGNN}~\cite{Fi-GNN} converts feature interactions into modeling node interactions on the graph for modeling feature interactions in an explicit way. \textbf{AutoInt}~\cite{AutoInt} adopts a self-attentive neural network with residual connections to model the feature interactions explicitly.

As fo reranking task, we implement the state-of-the-art models, \eg, \textbf{DLCM}~\cite{ai2018learning}, \textbf{PRM}~\cite{pei2019personalized}, \textbf{SetRank}~\cite{pang2020setrank}, and \textbf{MIR}~\cite{xi2022multi}, as backbone models. \textbf{DLCM} ~\cite{ai2018learning} first applies GRU to encode and rerank the top results. \textbf{PRM}~\cite{pei2019personalized} employs self-attention to model the mutual influence between any pair of items and users' preferences. \textbf{SetRank}~\cite{pang2020setrank} learns permutation-equivariant representations for the inputted items via self-attention. \textbf{MIR} \cite{xi2022multi} models the set-to-list interactions between candidate set and history list with personalized long-short term interests.

\subsubsection{PLM-based Baselines}
As for baselines, we compare REKA with methods that leverage pretrained language model to enhance recommendation, such as P5~\cite{p5}, UniSRec~\cite{UniSRec}, VQRec~\cite{VQRec}, TALLRec~\cite{bao2023tallrec}, and LLM2DIN~\cite{harte2023leveraging}. 
\textbf{P5}~\cite{p5} is a text-to-text paradigm that unifies recommendation tasks and learns different tasks with the same language modeling objective during pretraining. \textbf{UniSRec}~\cite{UniSRec} designs a universal sequence representation learning approach for sequential recommenders, which introduces contrastive pretraining tasks to effective transfer across scenarios. 
\textbf{VQ-Rec}~\cite{VQRec} uses Vector-Quantized item representations and a text-to-code-to-representation scheme, achieving effective cross-domain and cross-platform sequential recommendation. \textbf{TALLRec}~\cite{bao2023tallrec} finetunes LLaMa-7B~\cite{llama} with a LoRA architecture on recommendation tasks and enhances the recommendation capabilities of LLMs in few-shot scenarios. In our experiment, we implement TALLRec with LLaMa-2-7B-chat\footnote{https://huggingface.co/meta-llama/Llama-2-7b-chat-hf}, since it has better performance and ability of instruction following. According to~\cite{harte2023leveraging}, we design \textbf{LLM2DIN} which initializes DIN with item
embeddings obtained from chatGLM\cite{du2022glm}. We utilize the publicly available code of these three models and adapt the model to the CTR task with necessary minor modifications. We also align the data and features for all the methods to ensure fair comparisons.
% Based on T5~\cite{t5}, \textbf{P5}~\cite{p5} learns different recommendation tasks with the same language modeling objective. \textbf{UniSRec}~\cite{UniSRec} learns a universal sequence representation for sequential recommenders, with  contrastive sequence pretraining tasks and representations from BERT. 
% \textbf{VQ-Rec}~\cite{VQRec} builds upon UniSRec and uses Vector-Quantized item representations to achieve cross-domain and cross-platform sequential recommendation. We utilize the publicly available code of these three models and adapt the model to the CTR task with necessary minor modifications. We also align the data and features for all the methods to ensure fair comparisons.


% 
% \smallskip
% \noindent
% \textbf{Feature Interaction Models} focus on modeling feature interactions between different feature fields. \textbf{DeepFM}~\cite{DeepFM} is a classic CTR model that combines factorization machine (FM) and neural network to capture low-order and high-order feature interactions. \textbf{xDeepFM} \cite{xDeepFM} leverages the power of both deep network and Compressed Interaction Network to generate feature interactions at the vector-wise level. \textbf{DCN}~\cite{DCN} incorporates cross-network architecture and the DNN model to learn the bounded-degree feature interactions. \textbf{DCNv2}~\cite{DCNv2} is an improved framework of DCN which is more practical in large-scale industrial settings. \textbf{FiBiNet}~\cite{FiBiNET} can dynamically learn the feature importance by Squeeze-Excitation network and fine-grained feature interactions by bilinear function. \textbf{FiGNN}~\cite{Fi-GNN} converts feature interactions into modeling node interactions on the graph for modeling feature interactions in an explicit way. \textbf{AutoInt}~\cite{AutoInt} adopts a self-attentive neural network with residual connections to explicitly model the feature interactions.

% % \smallskip
% % \noindent
% \textbf{User Behavior Models} emphasize on modeling sequential dependencies of user behaviors. \textbf{DIN}~\cite{DIN} utilizes attention to model user interests dynamically with respect to a certain item. \textbf{DIEN}~\cite{DIEN} extends DIN by introducing an interest evolving mechanism to capture the dynamic evolution of user interests over time. 
% % On the other hand, models focusing on user behavior modeling include DIN and DIEN. 
% % Backbone Models
% % \begin{itemize}
% %     \item DeepFM \cite{DeepFM}
% %     \item xDeepFM \cite{xDeepFM}
% %     \item DCN \cite{DCN}
% %     \item DCNv2 \cite{DCNv2}
% %     \item FiBiNET \cite{FiBiNET}
% %     \item Fi-GNN \cite{Fi-GNN}
% %     \item AutoInt \cite{AutoInt}
% %     \item DIN \cite{DIN}
% %     \item DIEN \cite{DIEN}
% % \end{itemize}

% \subsubsection{Pretraining Baselines}
% We compare REKA with some baselines that leverage pretraining techniques with text or behavioral data to enhance the recommendation models, such as P5~\cite{p5}, UniSRec~\cite{UniSRec}, VQRec~\cite{VQRec}. \textbf{P5}~\cite{p5} is a text-to-text paradigm that unifies recommendation tasks and learns different tasks with the same language modeling objective during pretraining. \textbf{UniSRec}~\cite{UniSRec} designs a universal sequence representation learning approach for sequential recommenders, which  introduces contrastive pretraining tasks to effective transfer across scenarios. 
% \textbf{VQ-Rec}~\cite{VQRec} uses Vector-Quantized item representations and a text-to-code-to-representation scheme, achieving effective cross-domain and cross-platform sequential recommendation. We utilize the publicly available code of these three models and adapt the model to the CTR task with necessary minor modifications. We also align the data and features for all the methods to ensure fair comparisons.

\subsubsection{Evaluation Metrics} On CTR prediction task, we employ widely-used \textit{AUC} (Area under the ROC curve) and \textit{LogLoss} (binary cross-entropy loss) as evaluation metrics following~\cite{DCNv2,AutoInt,DeepFM,DIN}. A higher AUC value or a lower Logloss value, even by a small margin (\eg, 0.001), can be viewed as a significant improvement in CTR prediction performance, as indicated by previous studies~\cite{xDeepFM,DCNv2}. As for reranking task, several widely used metrics, \textit{NDCG@K}~\cite{ndcg} and \textit{MAP@K}~\cite{yue2007support}, are adopted, following previous work~\cite{xi2022multi,ai2018learning,pei2019personalized}.
% A higher AUC value or a lower Logloss value, even by a small margin (e.g., 0.001), can be considered as a significant improvement in CTR prediction performance, as indicated by previous studies~\cite{xDeepFM,DCNv2}.
% \Jianghao{the last sentence is unnecessary actually}

\subsubsection{Implementation Details} 
We utilize ChatGPT\footnote{\url{https://openai.com/product/chatgpt}} (gpt-3.5-turbo) from OpenAI as the LLM to generate the knowledge we need. During our experiment, we utilized approximately 33,000 knowledge messages\footnote{All this knowledge is available at  \url{https://github.com/YunjiaXi/Open-World-Knowledge-Augmented-Recommendation}} generated by ChatGPT, with an average token length of around 550. And the total cost is about \$150, including some preliminary exploratory experiments.
% We utilize API of a widely-used LLM for generating reasoning and factual knowledge. 
In the previous methods, we have designed two approaches for knowledge generation: generating individual knowledge for each item and user (referred to as \textbf{REKA-I}  in experiments) and clustering items and users before generating collective knowledge for each cluster (referred to as \textbf{REKA-C} in experiments). Apart from the difference in knowledge generation, the encoders for REKA-I and REKA-C in the experimental section are also different. Unless explicitly stated, REKA-I employs ChatGLM-6B as the encoder, while REKA-C uses BERT as the encoder. We will explain the reason for this choice and compare the performance of two variants in Section~\ref{sec:infer_compar}. Besides, to compensate for the lack of individual information in REKA-C, we also utilize the same encoder to encode the recent history of each user and the descriptions of items as additional augmented vectors. If not specified, REKA generally represents REKA-I.
Then, after the encoder, the average pooling is utilized as the aggregation function in Eq.~\eqref{eq:aggr_encoder}. Each expert in the hybrid-expert adaptor is implemented as an MLP with a hidden layer size of [128, 32]. The number of experts varies slightly across different backbone models, typically with 2-5 shared experts and 2-6 dedicated experts. We keep the embedding size of the backbone model as 32, and the output layer MLP size as [200, 80]. Other parameters, such as batch size and learning rate, are determined through grid search to achieve the best results. For fair comparisons, the parameters of the backbone model and the baselines are also tuned to achieve their optimal performance.
% Due to the unavailability of ChatGPT's parameters,
% The implementation of our proposed REKA is publicly available~\footnote{Our code is available at \url{https://anonymous.4open.science/r/REKA-8FAC}}.
% To further optimize the API cost, we partition the user's whole behavior sequence into several segments and use the most recent segment preceding the target item as the user history in the preference reasoning prompt. In this way, we can avoid the frequent API calls and significantly reduce the computational overhead.

 % instead of using the behaviors before the current sample as the user history in the preference reasoning prompt,
% For example, suppose the user's whole behavior sequence contains 100 items $h_1-h_{100}$, which can be divided into 4 segments. Then the target item from $h_{26}$ to $h_{49}$ will all share the same user history of $h_1-h_{25}$. In this way, we can avoid the frequent API calls and significantly reduce the computational overhead.

% If the target item is $h_{30}$, the segment $h_1-h_{25}$ will be used for preference reasoning. 
% In practice, the major cost of calling API comes from inferring user preferences based on user behaviors, since each click record corresponds to a unique user history. For example, MovieLens-1M contains 1 million click records for only 4000 movies. Considering LLMs can focus on long-term preferences rather than relying on recent behaviors, we can partition the user history into several segments and use the most recent segment preceding the target item. For example, there are 100 items $h_1-h_{100}$ in user history which can be divided into 4 segments. If the target item is $h_{30}$, the segment $h_1-h_{20}$ will be used for preference reasoning. By calling the API only once for each historical segments, we can significantly reduce the computional overhead.



\begin{table*}[h]
\centering
% \vspace{-4pt}
\caption{Comparison between REKA and backbone CTR prediction models.}
% \vspace{-4pt}
\scalebox{0.88}{
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{ccccccc|cccccc}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Backbone\\ model\end{tabular}}} & \multicolumn{6}{c|}{\textbf{MovieLens-1M}} & \multicolumn{6}{c}{\textbf{Amazon-Books}} \\
\cmidrule{2-13}
%  & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c|}{\textbf{LogLoss}} & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{LogLoss}} \\
%  \cmidrule{2-13}
%  & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.}  \\
%  \midrule
% DCNv2 & 0.7924 & \textbf{0.8049*} & 1.58\% & 0.5451 & \textbf{0.5315*} & 2.50\% & 0.8269 & \textbf{0.8350*} & 0.98\% & 0.4973 & \textbf{0.4865*} & 2.17\% \\
% DCNv1 & 0.7929 & \textbf{0.8044*} & 1.46\% & 0.5457 & \textbf{0.5319*} & 2.53\% & 0.8268 & \textbf{0.8348*} & 0.97\% & 0.4973 & \textbf{0.4869*} & 2.11\% \\
% DeepFM & 0.7928 & \textbf{0.8041*} & 1.44\% & 0.5462 & \textbf{0.5321*} & 2.57\% & 0.8269 & \textbf{0.8347*} & 0.94\% & 0.4969 & \textbf{0.4873*} & 1.93\% \\
% FiBiNet & 0.7925 & \textbf{0.8051*} & 1.59\% & 0.5450 & \textbf{0.5310*} & 2.56\% & 0.8269 & \textbf{0.8351*} & 0.99\% & 0.4973 & \textbf{0.4870*} & 2.07\% \\
% AutoInt & 0.7934 & \textbf{0.8060*} & 1.59\% & 0.5440 & \textbf{0.5297*} & 2.65\% & 0.8262 & \textbf{0.8357*} & 1.16\% & 0.4981 & \textbf{0.4863*} & 2.37\% \\
% FiGNN & 0.7944 & \textbf{0.8054*} & 1.39\% & 0.5424 & \textbf{0.5307*} & 2.16\% & 0.8270 & \textbf{0.8352*} & 0.99\% & 0.4977 & \textbf{0.4870*} & 2.14\% \\
% xDeepFM & 0.7942 & \textbf{0.8041*} & 1.25\% & 0.5457 & \textbf{0.5317*} & 2.57\% & 0.8271 & \textbf{0.8351*} & 0.97\% & 0.4971 & \textbf{0.4866*} & 2.10\% \\
% DIEN & 0.7960 & \textbf{0.8059*} & 1.25\% & 0.5469 & \textbf{0.5298*} & 3.13\% & 0.8307 & \textbf{0.8391*} & 1.01\% & 0.4926 & \textbf{0.4812*} & 2.32\% \\
% DIN & 0.7975 & \textbf{0.8066*} & 1.15\% & 0.5387 & \textbf{0.5304*} & 1.55\% & 0.8304 & \textbf{0.8418*} & 1.38\% & 0.4937 & \textbf{0.4801*} & 2.77\%\\
%  & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c|}{\textbf{LogLoss}} & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{LogLoss}} \\
%  \cmidrule{2-13}
%  & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.}  \\
%  \midrule
% DCNv2                                                                              & 0.7830          & \textbf{0.7935*} & 1.34\%           & 0.5516          & \textbf{0.5410*} & 1.92\%           & 0.8269        & \textbf{0.8350*} & 0.98\%           & 0.4973        & \textbf{0.4865*} & 2.17\%           \\
% DCNv1                                                                              & 0.7828          & \textbf{0.7927*} & 1.28\%           & 0.5528          & \textbf{0.5411*} & 2.12\%           & 0.8268        & \textbf{0.8348*} & 0.97\%           & 0.4973        & \textbf{0.4869*} & 2.11\%           \\
% DeepFM                                                                             & 0.7824 & \textbf{0.7919*} & 1.22\%           & 0.5518 & \textbf{0.5432*} & 1.56\%  & 0.8269        & \textbf{0.8347*} & 0.94\%           & 0.4969        & \textbf{0.4873*} & 1.93\%           \\
% FiBiNet                                                                            & 0.7820          & \textbf{0.7936*} & 1.49\%           & 0.5531          & \textbf{0.5405*} & 2.27\%           & 0.8269        & \textbf{0.8351*} & 0.99\%           & 0.4973        & \textbf{0.4870*} & 2.07\%           \\
% AutoInt                                                                            & 0.7821          & \textbf{0.7931*} & 1.40\%           & 0.5520          & \textbf{0.5430*} & 1.62\%           & 0.8262        & \textbf{0.8357*} & 1.16\%           & 0.4981        & \textbf{0.4863*} & 2.37\%           \\
% FiGNN                                                                              & 0.7832          & \textbf{0.7935*} & 1.32\%           & 0.5510          & \textbf{0.5437*} & 1.33\%           & 0.8270        & \textbf{0.8352*} & 0.99\%           & 0.4977        & \textbf{0.4870*} & 2.14\%           \\
% xDeepFM                                                                            & 0.7823          & \textbf{0.7926*} & 1.32\%           & 0.5520          & \textbf{0.5420*} & 1.81\%           & 0.8271        & \textbf{0.8351*} & 0.97\%           & 0.4971        & \textbf{0.4866*} & 2.10\%           \\
% DIEN                                                                               & 0.7853          & \textbf{0.7953*} & 1.27\%           & 0.5494          & \textbf{0.5394*} & 1.83\%           & 0.8307        & \textbf{0.8391*} & 1.01\%           & 0.4926        & \textbf{0.4812*} & 2.32\%           \\
% DIN                                                                                & 0.7863          & \textbf{0.7961*} & 1.24\%           & 0.5486          & \textbf{0.5370*} & 2.10\%           & 0.8304        & \textbf{0.8418*} & 1.38\%           & 0.4937        & \textbf{0.4801*} & 2.77\%          \\
 & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c|}{\textbf{Logloss}} & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{Logloss}} \\
  \cmidrule{2-13}
 & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} \\
 \midrule
DCNv2 & 0.7830 & 0.7918 & \textbf{0.7935} & 0.5516 & 0.5432 & \textbf{0.5410} & 0.8269 & 0.8345 & \textbf{0.8350} & 0.4973 & 0.4871 & \textbf{0.4865} \\
DCNv1 & 0.7828 & 0.7918 & \textbf{0.7931} & 0.5528 & 0.5428 & \textbf{0.5411} & 0.8268 & 0.8342 & \textbf{0.8348} & 0.4973 & 0.4878 & \textbf{0.4869} \\
DeepFM & 0.7824 & \textbf{0.7920} & 0.7919 & 0.5518 & 0.5429 & \textbf{0.5432} & 0.8269 & 0.8341 & \textbf{0.8347} & 0.4969 & 0.4889 & \textbf{0.4873} \\
FiBiNet & 0.7820 & 0.7925 & \textbf{0.7938} & 0.5531 & 0.5422 & \textbf{0.5405} & 0.8269 & 0.8342 & \textbf{0.8351} & 0.4973 & 0.4882 & \textbf{0.4870} \\
AutoInt & 0.7821 & 0.7918 & \textbf{0.7935} & 0.5520 & 0.5427 & \textbf{0.5405} & 0.8262 & 0.8344 & \textbf{0.8357} & 0.4981 & 0.4873 & \textbf{0.4863} \\
FiGNN & 0.7832 & 0.7923 & \textbf{0.7935} & 0.5510 & \textbf{0.5431} & 0.5437 & 0.8270 & 0.8345 & \textbf{0.8352} & 0.4977 & 0.4888 & \textbf{0.4870} \\
xDeepFM & 0.7823 & 0.7924 & \textbf{0.7934} & 0.5520 & 0.5430 & \textbf{0.5428} & 0.8271 & 0.8344 & \textbf{0.8351} & 0.4971 & 0.4869 & \textbf{0.4866} \\
DIEN & 0.7853 & 0.7944 & \textbf{0.7953} & 0.5494 & 0.5395 & \textbf{0.5394} & 0.8307 & 0.8374 & \textbf{0.8391} & 0.4926 & 0.4851 & \textbf{0.4812} \\
DIN & 0.7863 & 0.7952 & \textbf{0.7961} & 0.5486 & 0.5398 & \textbf{0.5370} & 0.8304 & 0.8396 & \textbf{0.8418} & 0.4937 & 0.4808 & \textbf{0.4801} \\
\bottomrule
\end{tabular}
}
}
\footnotesize \flushleft\hspace{0.0cm} $*$ denotes statistically significant improvement over backbone CTR prediction models (t-test with $p$-value $<$ 0.05).
% \vspace{-4pt}
\label{tab:backbone_model}
\end{table*}
\subsection{Effectiveness Comparison}
\subsubsection{Improvement over Backbone Models (RQ1)} On \textbf{CTR prediction} task, we implement our proposed REKA-I and REKA-C upon 9 representative CTR models, and the results are shown in Table~\ref{tab:backbone_model}. From the table, we can have the following observations: \textbf{(i)} Applying REKA significantly improves the performance of backbone CTR models. For example, when using FiBiNet as the backbone model on MovieLens-1M, REKA-I achieves a 1.49\% increase in AUC and a 2.27\% decrease in LogLoss, demonstrating the effectiveness of incorporating open-world knowledge from LLMs into RSs. \textbf{(ii)} As a model-agnostic framework, REKA can be applied to various types of baseline models, whether focusing on feature interaction or behavior modeling. With the equipment of REKA-I, the selected 9 representative CTR models on two datasets all achieve an AUC improvement of about 1-1.5\%, indicating the universality of the REKA. \textbf{(iii)} REKA-I and REKA-C show more remarkable improvement in feature interaction models compared to user behavior models. This may be because the knowledge augmented vectors generated by REKA are utilized more effectively by the feature interaction layer than the user behavior modeling layer. The dedicated feature interaction design may better exploit the information contained in the knowledge vectors. \textbf{(iv)} Generally, in CTR tasks, REKA-C exhibits a performance decrease of 0.1\% - 0.2\% compared to REKA-I. This is because using REKA-C with clustered collective knowledge may result in some information loss compared to individual knowledge generated for each user. However, relative to REKA-I, REKA-C can significantly reduce the time required for the knowledge generation, training, and inference time of the backbone model, as presented in Section~\ref{sec:infer_compar}. Therefore, considering the substantial improvement in efficiency, such a level of accuracy loss is acceptable.



% \begin{table*}[]
% \centering
% \vspace{-8pt}
% \caption{Comparison between REKA and backbone models.}
% \vspace{-5pt}
% \scalebox{1.0}{
% \setlength{\tabcolsep}{1.5mm}{
% \begin{tabular}{cccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}backbone\\ model\end{tabular}}} & \multicolumn{6}{c|}{\textbf{MovieLens-1M}} & \multicolumn{6}{c}{\textbf{Amazon-Books}} \\
%  \cmidrule{2-13}
%  & \multicolumn{3}{c|}{\textbf{AUC}} & \multicolumn{3}{c|}{\textbf{LogLoss}} & \multicolumn{3}{c|}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{LL}} \\
%   \cmidrule{2-13}
%  & \textbf{base} & \textbf{REKA} & \textbf{improv.} & \textbf{base} & \textbf{REKA} & \textbf{improv.} & \textbf{base} & \textbf{REKA} & \textbf{improv.} & \textbf{base} & \textbf{REKA} & \textbf{improv.} \\
%  \midrule
% DCNv2 & 0.7924 & \textbf{0.8049*} & 1.58\% & 0.5451 & \textbf{0.5315*} & 2.50\% & 0.8269 & \textbf{0.8350*} & 0.98\% & 0.4973 & \textbf{0.4865*} & 2.17\% \\
% DCNv1 & 0.7929 & \textbf{0.8044*} & 1.46\% & 0.5457 & \textbf{0.5319*} & 2.53\% & 0.8268 & \textbf{0.8348*} & 0.97\% & 0.4973 & \textbf{0.4869*} & 2.11\% \\
% DeepFM & 0.7928 & \textbf{0.8041*} & 1.44\% & 0.5462 & \textbf{0.5321*} & 2.57\% & 0.8269 & \textbf{0.8347*} & 0.94\% & 0.4969 & \textbf{0.4873*} & 1.93\% \\
% FiBiNet & 0.7925 & \textbf{0.8051*} & 1.59\% & 0.5450 & \textbf{0.5310*} & 2.56\% & 0.8269 & \textbf{0.8351*} & 0.99\% & 0.4973 & \textbf{0.4870*} & 2.07\% \\
% AutoInt & 0.7934 & \textbf{0.8060*} & 1.59\% & 0.5440 & \textbf{0.5297*} & 2.65\% & 0.8262 & \textbf{0.8357*} & 1.16\% & 0.4981 & \textbf{0.4863*} & 2.37\% \\
% FiGNN & 0.7944 & \textbf{0.8054*} & 1.39\% & 0.5424 & \textbf{0.5307*} & 2.16\% & 0.8270 & \textbf{0.8352*} & 0.99\% & 0.4977 & \textbf{0.4870*} & 2.14\% \\
% xDeepFM & 0.7942 & \textbf{0.8041*} & 1.25\% & 0.5457 & \textbf{0.5317*} & 2.57\% & 0.8271 & \textbf{0.8351*} & 0.97\% & 0.4971 & \textbf{0.4866*} & 2.10\% \\
% DIEN & 0.7960 & \textbf{0.8059*} & 1.25\% & 0.5469 & \textbf{0.5298*} & 3.13\% & 0.8307 & \textbf{0.8391*} & 1.01\% & 0.4926 & \textbf{0.4812*} & 2.32\% \\
% DIN & 0.7975 & \textbf{0.8066*} & 1.15\% & 0.5387 & \textbf{0.5304*} & 1.55\% & 0.8304 & \textbf{0.8418*} & 1.38\% & 0.4937 & \textbf{0.4801*} & 2.77\% \\
% \bottomrule
% \end{tabular}
% }
% }
% \footnotesize \flushleft\hspace{0.3cm} $*$ denotes statistically significant improvement (t-test with $p$-value $<$ 0.05) over the backbone model.
% \vspace{-0pt}
% \label{tab:backbone_model}
% \end{table*}

To investigate REKA's compatibility on other tasks, \eg, \textbf{reranking}, we incorporate REKA into the state-of-the-art reranking models. The results on the Amazon-Books dataset are presented in Table ~\ref{tab:reranking}, from which the following observations can be made: \textbf{(i)} REKA significantly enhances the performance of backbone reranking models. For example, when PRM is employed as the backbone, REKA-I achieves a remarkable increase of 5.71\% and 4.71\% in MAP@7 and NDCG@7. \textbf{(ii)} REKA demonstrates more pronounced improvements in methods that do not involve history modeling, such as DLCM, PRM, and SetRank. The user preference knowledge provided by REKA is particularly advantageous for these methods. However, in MIR, which adequately explores the relationship between history and candidates, the enhancement is slightly smaller. \textbf{(iii)} The performance of REKA-C and REKA-I on reranking tasks is similar to that on CTR tasks, with REKA-I generally performing slightly better than REKA-C. However, this effect is also influenced by the backbone model and may exhibit some exceptions. For example, when using DLCM as the backbone model, REKA-C performs better than REKA-I on the MovieLens-1M dataset.



\begin{table*}[h]
\centering
% \vspace{-5pt}
\caption{The comparison of REKA and backbone reranking models on MovieLens-1M dataset.}
% \vspace{-5pt}
\scalebox{0.88}{
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{ccccccc|cccccc}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Backbone\\ Model\end{tabular}}} & \multicolumn{3}{c}{\textbf{MAP@3}} & \multicolumn{3}{c|}{\textbf{MAP@7}} & \multicolumn{3}{c}
{\textbf{NDCG@3}} & \multicolumn{3}{c}{\textbf{NDCG@7}} \\
\cmidrule{2-13}
%  & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} & \textbf{base} & \textbf{REKA} & \textbf{Improv.} \\
%  \midrule
% DLCM & 0.6365 & \textbf{0.6654*} & 4.54\% & 0.6247 & \textbf{0.6512*} & 4.24\% & 0.5755 & \textbf{0.6109*} & 6.15\% & 0.6891 & \textbf{0.7142*} & 3.64\% \\
% PRM & 0.6488 & \textbf{0.6877*} & 6.00\% & 0.6359 & \textbf{0.6722*} & 5.71\% & 0.5909 & \textbf{0.6379*} & 7.95\% & 0.6983 & \textbf{0.7312*} & 4.71\% \\
% SetRank & 0.6509 & \textbf{0.6711*} & 3.10\% & 0.6384 & \textbf{0.6538*} & 2.41\% & 0.5947 & \textbf{0.6137*} & 3.19\% & 0.7006 & \textbf{0.7164*} & 2.26\% \\
% MIR & 0.7178 & \textbf{0.7241*} & 0.88\% & 0.7011 & \textbf{0.7078*} & 0.96\% & 0.6747 & \textbf{0.6837*} & 1.33\% & 0.7549 & \textbf{0.7597*} & 0.64\% \\
 & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} \\
 \midrule
DLCM & 0.7328 & \textbf{0.7508} & 0.7506 & 0.6899 & \textbf{0.7126} & 0.7100 & 0.7176 & \textbf{0.7353} & 0.7339 & 0.7766 & \textbf{0.7902} & 0.7899 \\
PRM & 0.7432 & 0.7521 & \textbf{0.7561} & 0.7029 & 0.714 & \textbf{0.7202} & 0.7285 & 0.7373 & \textbf{0.7418} & 0.7848 & 0.7923 & \textbf{0.7952} \\
SetRank & 0.7424 & 0.7554 & \textbf{0.7584} & 0.7037 & 0.7196 & \textbf{0.7238} & 0.7283 & 0.741 & \textbf{0.7443} & 0.7844 & 0.7943 & \textbf{0.7972} \\
MIR & 0.7629 & 0.7687 & \textbf{0.7696} & 0.7281 & 0.736 & \textbf{0.7372} & 0.7482 & 0.7551 & \textbf{0.7558} & 0.8006 & 0.8057 & \textbf{0.8066}\\
\bottomrule
\end{tabular}
}}
\label{tab:reranking}
% \vspace{-3}
\footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement over backbone reranking models (t-test with $p$-value $<$ 0.05).
\vspace{-5pt}
% \Jianghao{underline the second best value}
\end{table*}

\begin{table*}[h]
\centering
% \vspace{-5pt}
\caption{The comparison of REKA and backbone reranking models on Amazon-Books dataset.}
% \vspace{-5pt}
\scalebox{0.88}{
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{ccccccc|cccccc}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Backbone\\ Model\end{tabular}}} & \multicolumn{3}{c}{\textbf{MAP@3}} & \multicolumn{3}{c|}{\textbf{MAP@7}} & \multicolumn{3}{c}
{\textbf{NDCG@3}} & \multicolumn{3}{c}{\textbf{NDCG@7}} \\
\cmidrule{2-13}
 & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} & \textbf{base} & \textbf{REKA-C} & \textbf{REKA-I} \\
 \midrule
DLCM & 0.6365 & 0.6651 & \textbf{0.6654} & 0.6247 & 0.6488 & \textbf{0.6512} & 0.5755 & 0.6075 & \textbf{0.6109} & 0.6891 & 0.713 & \textbf{0.7142} \\
PRM & 0.6488 & 0.6738 & \textbf{0.6877} & 0.6359 & 0.6583 & \textbf{0.6722} & 0.5909 & 0.6191 & \textbf{0.6379} & 0.6983 & 0.7201 & \textbf{0.7312} \\
SetRank & 0.6509 & \textbf{0.6725} & 0.6711 & 0.6384 & \textbf{0.6573} & 0.6538 & 0.5947 & \textbf{0.6183} & 0.6137 & 0.7006 & \textbf{0.7191} & 0.7164 \\
MIR & 0.7178 & 0.7233 & \textbf{0.7241} & 0.7011 & 0.7069 & \textbf{0.7078} & 0.6747 & 0.6817 & \textbf{0.6837} & 0.7549 & 0.7591 & \textbf{0.7597} \\
\bottomrule
\end{tabular}
}}
\label{tab:reranking}
\footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement over backbone reranking models (t-test with $p$-value $<$ 0.05).
\vspace{-5pt}
\end{table*}



\subsubsection{Improvement over Baselines (RQ2)} Next, we compare REKA with recent baselines using language models or sequence representation pretraining on CTR task. The results are presented in Table~\ref{tab:baselines}, from which we make the following observations: \textbf{(i)} REKA significantly outperforms models based on pretrained language models. For instance, with DIN as the backbone on Amazon-Books, REKA-I achieves a 0.91\% improvement in AUC and a 1.27\% improvement in LogLoss over the strongest baseline TALLRec. This validate the effectiveness of incorporation between LLMs and CRMs.
\textbf{(ii)} When integrating PLMs into RSs, the improvements brought by smaller PLMs are relatively modest. For instance, UniSRec, VQ-Rec, and P5, based on PLMs with parameters less than one billion, tend to exhibit poorer performance, even worse than the baseline DIN. \textbf{(iii)} Conversely, leveraging LLMs can lead to more substantial improvements, as seen in TALLRec and REKA. However, achieving effective enhancements with LLM embedding as initialization proves challenging, \eg, there is little difference between the results of LLM2DIN and DIN.

% (ii) Pretraining models such as UniSRec, VQ-Rec and P5, perform poorly, and even fail to surpass the basic DIN. This could be attributed to the fact that the those studies has little exploration of the feature interaction, while the CTR prediction heavily relies on feature interaction.


% ~\footnote{We did not include the results of P5, because when adapting its official code to CTR task, its metrics are notably worse than others even after careful parameter tuning. \xx{For instance, on MovieLens-1M, the AUC for P5 is only 0.713, significantly worse than other baselines. This may be attributed to the fact that CTR tasks heavily rely on feature interaction, while language models like P5 struggle to capture this effectively.}}
% (iii) P5 (to be completed)
\begin{table}[h]
\centering
% \vspace{-5pt}
\caption{Comparison between REKA and baselines. }
% \vspace{-5pt}
\scalebox{1.0}{
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Backbone\\ PLM\end{tabular}}}& \multicolumn{2}{c|}{\textbf{MovieLens-1M}} & \multicolumn{2}{c}{\textbf{Amazon-Books}} \\
\cmidrule{3-6}
 & & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} \\
 \midrule
% UniSRec & BERT-110M & 0.7891 & 0.5496 & 0.8196 & 0.5063 \\
% VQ-Rec & BERT-110M & 0.7914 & 0.5456 & 0.8226 & 0.5025 \\
% P5& T5-223M & 0.7935 & 0.5436 & 0.8333 & 0.4908 \\
% LLM2DIN & ChatGLM-6B & 0.7977 & 0.5379 & 0.8307 & 0.4930  \\
% TALLRec & LLaMA2-7B & \underline{0.8007} & \underline{0.5372} & \underline{0.8342} & \underline{0.4862}  \\
% base(DIN) &N/A & 0.7975 & 0.5387 & 0.8304 & 0.4937 \\
% REKA(DIN) &gpt-3.5-turbo & \textbf{0.8066*} & \textbf{0.5304*} & \textbf{0.8418*} & \textbf{0.4801*} \\
UnisRec                         & BERT-110M                                                                         & 0.7702              & 0.5641              & 0.8196              & 0.5063              \\
VQ-Rec                          & BERT-110M                                                                         & 0.7707              & 0.5641              & 0.8226              & 0.5025              \\
P5                              & T5-223M                                                                           & 0.7790              & 0.5543              & 0.8333              & 0.4908              \\
LLM2DIN                         & ChatGLM-6B                                                                        & 0.7874              & 0.5473              & 0.8307              & 0.4930              \\
TALLRec                         & LLaMa2-7B                                                                         & \underline{0.7892}        & \underline{0.5451}        & \underline{0.8342}        & \underline{0.4862}        \\
base(DIN)                       & N/A                                                                               & 0.7863              & 0.5486              & 0.8304              & 0.4937              \\
REKA-C(DIN)                        & gpt-3.5-turbo                                                                        & \textbf{0.7952*}    & \textbf{0.5398*}    & \textbf{0.8396*}    & \textbf{0.4808*}   \\
REKA-I(DIN)                        & gpt-3.5-turbo                                                                        & \textbf{0.7961*}    & \textbf{0.5370*}    & \textbf{0.8418*}    & \textbf{0.4801*}   \\
\bottomrule
\end{tabular}
}}
\label{tab:baselines}
\footnotesize \flushleft\hspace{3cm} $*$ denotes statistically significant improvement over the second best baselines which is \\\flushleft\hspace{3cm}underlined (t-test with $p$-value $<$ 0.05).
\vspace{-5pt}
% \Jianghao{underline the second best value}
\end{table}

% \subsubsection{Generalization on Other Task (RQ3)} 

\subsubsection{Improvement over Other Knowledge (RQ3)} Finally, in Figure~\ref{fig:kge}, we compare knowledge from LLMs and other sources, such as knowledge graph (KG),  with DCNv1, DeepFM, and DIN as the backbone on MovieLens-1M dataset. We utilize a knowledge graph from LODrecsys~\cite{DOTD16}, which maps items of MovieLens-1M to DBPedia entities. Then, the entity embedding of each item is extracted following KTUP~\cite{cao2019unifying} and used as an additional feature for the backbone model. The legend ``\textbf{None}" denotes the backbone model without knowledge enhancement, while ``\textbf{KG}", ``\textbf{LLM}", and ``\textbf{Both}" represent the backbone model enhanced by knowledge from KG, LLM, and both sources, respectively. Note that the individual knowledge generated in \textbf{REKA-I} is utilized for \textbf{LLM}.

\begin{figure}[h]
    \centering
% \vspace{-7pt}
    \includegraphics[width=0.65\textwidth]{imgs/kge_new.pdf}
% \vspace{-6pt}
    \caption{Comparison between knowledge from knowledge graph and LLM on MovieLens-1M dataset.}
\vspace{-5pt}
    \label{fig:kge}
\end{figure}


From Figure~\ref{fig:kge}, we notice that knowledge from both KG and LLM can bring performance improvements; however, the enhancement of KG is much smaller compared to that of LLM. This might be attributed to the fact that KG only possesses manually annotated item-side knowledge while it lacks knowledge for user preferences. According to our analysis in the next subsection~\ref{reas_fact_konwledge}, the knowledge for user preference usually contributes more gains compared to item factual knowledge. Furthermore, the simultaneous utilization of the two kinds of knowledge does not exhibit significant improvement over using LLM alone. This suggests that LLM may already encompass the typical knowledge within KG, making knowledge derived solely from LLM sufficient. 

\subsection{Deployment \& Online A/B Test (RQ4)}\label{sec:online}
\subsubsection{System Design}
In this section, we briefly introduce the system design of REKA during the deployment process, as illustrated in Figure~\ref{fig:system}. The entire system consists of two phases: the offline training phase and the online inference phase. The offline phase involves the knowledge generation of LLM and the training of conventional recommendation model (CRM). During the knowledge generation, we extract features correspond to users and items  from the feature database based on the requirements of the scenario, which are used to construct prompts for LLM. Then the LLM is employed to generate respective knowledge for users and items. Subsequently, a smaller language model encodes the generated knowledge into knowledge representations. These representations are stored in the knowledge database for subsequent training and inference of the CRM. In the offline phase, we also conduct training for the CRM model. This process involves constructing training samples using the feature database and knowledge database and then completing the training. During the online inference phase, the CRM is deployed to the online system. The deployed CRM, along with data from the feature database and knowledge database, is utilized for inference, generating recommended results to users. User feedback is stored in the feature database for future training iterations.
\begin{figure}[h]
    \centering
% \vspace{-7pt}
    \includegraphics[width=0.8\textwidth]{imgs/system.pdf}
% \vspace{-6pt}
    \caption{The system design for the deployment of REKA.}
\vspace{-5pt}
    \label{fig:system}
\end{figure}
\subsubsection{Online A/B Test}
To validate the effectiveness of REKA, we conducted two online experiments on Huawei's news and music platforms, respectively. In the news scenario with a relatively small number of users, we extracted knowledge for each user and item, deploying REKA-I. In the music scenario involving a larger number of users and items, we adopt REKA-C for efficient knowledge reasoning and generation. REKA shows significant improvement over the original baselines on the online A/B test for both scenarios. Now, REKA has already been deployed online and serves the main traffic.

In Huawei's news scenario, we focus on the task of news recall, for which we have adapted REKA-I into a recall model. During the knowledge reasoning and generation stage, we utilize Huawei's large language model PanGu\cite{zeng2021pangu} to generate knowledge. Initially, we provide the LLM with the titles of the 20 most recently clicked news articles by a user. With the coarse-grained new categories, such as sports, finance, society, technology, etc., as scenario-specific factors, the LLM is required to infer the user's fine-grained preferences within those news categories. Once we obtain the user's fine-grained preferences, another smaller language model, all-MiniLM-L12-v2\footnote{https://huggingface.co/sentence-transformers/all-MiniLM-L12-v2}, encodes those preferences and candidate news articles. Those encodings are then used to calculate similarity scores, and news articles with higher similarity scores will be retrieved. The experimental group has been deployed the aforementioned version of REKA-I, while the control group utilizes the original recall model as our baseline. During the online A/B test, REKA exhibited a 7\% improvement on the Recall metric compared with the baseline, resulting in significant business benefits. 
% We randomly divided 50\% of users into experimental group, and the remaining 50\% were assigned to the control group. The experimental group used knowledge vectors generated by REKA for recall, while the control group utilized the original recall model as our baseline. 

In the music scenario, we utilize REKA for the CTR prediction task, which we have mentioned in our experiments. This scenario involves a larger number of users and items, leading us to adopt REKA-C. In this scenario, 30\% of users were randomly selected into the experimental group, and another 30\% were in the control group. Both groups used the same base model for generating recommendations. The difference lies in their inputs, where the input of the experimental group included the knowledge representation augmented by REKA-C. In large-scale domains, storage efficiency is also a crucial aspect that we need to consider. Therefore, we employ Principal Component Analysis (PCA) to reduce the dimension of knowledge representations to 64 and store them in a vector database. Additionally, we adopt incremental update, which only processes the updated items and users daily and adds them to the vector database. In a 7-day online A/B test, REKA demonstrated a 1.99\% increase in song play count, a 1.73\% increase in the number of devices for song playback, and a 2.04\% increase in total duration. Now, REKA has already been deployed online and serves the main traffic in this scenario. This indicates that REKA can be successfully implemented in industrial settings and improve the recommendation experience for real-world users. 

% \ww{This part is too short, could add a flowchart for online deployment.}
% The experimental group received recommendation generated by a base model with vectors augmented by LLM, i.e., REKA, while the control group did not incorporate this enhancement.

% \vspace{-7pt}
\subsection{Efficiency Study (RQ5)}\label{sec:efficiency}
\subsubsection{Offline Efficiency}\label{sec:infer_compar}
To study the offline efficiency of our proposed model, we first compared the performance and efficiency of two variants of REKA, namely \textbf{REKA-I} and \textbf{REKA-C}, which utilize individual and collective forms of knowledge, respectively, with base model DIN and the strongest baseline TALLREC. REKA-I requires generating individual knowledge using LLM for each item and user, while REKA-C generates collective knowledge for clusters of items and users, reducing the number of knowledge generations. For both REKA-I and REKA-C, we employ three different sizes of encoders: ChatGLM-6B, BERT-110M, and tinyBERT-14.7M. Regarding offline efficiency, we compared the number of knowledge generation calls for the entire dataset (\textbf{\# call} in the table) and the training time per batch for each model, which can be regarded as measures of offline resource consumption (both time and computational resource). For REKA-I and REKA-C, \textbf{\# call} represents the number of knowledge generation calls on ChatGPT API. For baseline TALLREC, \textbf{\# call} denotes the number of times the LLM is invoked to generate the final CTR predictions, corresponding to the sum of training and testing data samples. All experiments in Table~\ref{tab:inference_comp} are conducted on the same Tesla V100 with 32GB memory, and the batch size of training are set to 256. The only exception is that the GPU memory size limitation prevents us from setting the batch size of TALLREC to 256, so we present the training  time with the batch size set to 1. From these experiments, we draw the following conclusions.

\begin{table*}[h]
\centering
% \vspace{-5pt}
\caption{Offline efficiency comparison amongst variants of REKA and baselines.}
% \vspace{-5pt}
\scalebox{0.9}{
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{cccccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Encoder}} & \multicolumn{4}{c|}{\textbf{MovieLens-1M}} & \multicolumn{4}{c}{\textbf{Amazon-books}} \\
\cmidrule{3-10}
 &  & \textbf{\# call} & \textbf{training time (s)} & \textbf{AUC} & \textbf{Logloss} & \textbf{\# call} & \textbf{training time (s)} & \textbf{AUC} & \textbf{Logloss} \\
 \midrule
\textbf{DIN} & / & / & $8.41\times10^{-3}$ & 0.7863 & 0.5486 & / & $1.46\times10^{-2}$ & 0.8304 & 0.4937 \\
\textbf{TALLREC} & / & 167167 & $9.76\times10^{-1}$ & 0.7892 & 0.5451 & 268029 & $8.91\times10^{-1}$ & 0.8342 & 0.4862 \\
\midrule
\multirow{3}{*}{\textbf{KAR-I}} & \textbf{ChatGLM-6B} & 9923 & $9.59\times10^{-2}$ & 0.7961 & 0.5370 & 29238 & $9.68\times10^{-2}$ & 0.8418 & 0.4801 \\

 & BERT-110M & 9923 & $2.45\times10^{-2}$ & 0.7947 & 0.5412 & 29238 & $2.42\times10^{-2}$ & 0.8381 & 0.4839 \\
 & tinyBERT-14.5M & 9923 & $1.48\times10^{-2}$ & 0.7907 & 0.5434 & 29238 & $1.47\times10^{-2}$ & 0.8358 & 0.4877 \\
 \bottomrule
\multirow{3}{*}{\textbf{KAR-C}} & ChatGLM-6B & 377 & $2.19\times10^{-1}$ & 0.7959 & 0.5387 & 2080 & $2.22\times10^{-1}$ & 0.8388 & 0.4814 \\
 & \textbf{BERT-110M} & 377 & $5.08\times10^{-2}$ & 0.7952 & 0.5398 & 2080 & $5.32\times10^{-2}$ & 0.8396 & 0.4808 \\
 & tinyBERT-14.5M & 377 & $2.77\times10^{-2}$ & 0.7928 & 0.5428 & 2080 & $2.75\times10^{-2}$ & 0.8378 & 0.4848\\
 \bottomrule
\end{tabular}
}}
\label{tab:inference_comp}
\end{table*}

Firstly, REKA demonstrates significantly higher efficiency in both time and computation resource consumption compared to approaches like TALLREC that directly utilize LLMs for recommendation. This efficiency arises from the fact that REKA-I only needs to generate knowledge for each user and item, whereas TALLREC needs to generate knowledge for all samples, and the quantity of samples is typically much larger than that of users and items. For instance, in the \textbf{\# call} metric of MovieLens-1M dataset, the knowledge generation frequency of REKA-I is one-sixteenth of TALLREC, which indicates that REKA-I incurs significantly fewer computational resources and less time consumption than TALLREC. Moreover, regarding both training times, REKA-I also outperforms TALLREC by a significant margin, roughly being only one-tenth of TALLREC. This also provides strong evidence of REKA's efficiency over TALLREC.

Secondly, for knowledge generation, collective knowledge extraction used by REKA-C effectively reduces the number of knowledge generation calls without losing much accuracy. For example, on MovieLens, \textbf{\# call} for REKA-C is one twenty-sixth of REKA-I, but the two variants show comparable prediction accuracy. Moreover, with more miniature encoders such as BERT and tinyBERT, REKA-C even outperforms REKA-I. Considering that knowledge generation involves larger language models, which are slower, using REKA-C can effectively improve the deployment efficiency of the model.

Lastly, with the same encoder, REKA-C exhibits longer training times compared to REKA-I, but REKA-C is more friendly to more miniature encoders. With the same encoder, REKA-C has approximately twice the training time of REKA-I, as REKA-C generates and utilizes more additional features. However, REKA-C is more friendly to smaller encoders. With encoders like BERT and tinyBERT, REKA-C exhibits an improvement over REKA-I, possibly because collective knowledge is more accessible for smaller encoders to comprehend. Therefore, in practical use, adopting REKA-C with a smaller encoder model, such as BERT, can lead to significant accelerations in knowledge generation and training time compared to REKA-I with ChatGLM, thereby enhancing model efficiency. This is why we employ ChatGLM-6B and BERT as default encoders for REKA-I and REKA-C in the preceding experiments.

\subsubsection{Inference Latency}\label{sec:speed_up_efficiency}
To quantify the actual inference latency of REKA and assess the effectiveness of the acceleration strategies, we compare the inference time of REKA-I based on DIN with ChatGPT API, strongest baseline TALLRec, and base DIN model in Table~\ref{tab:inference}. For \textbf{ChatGPT API}, we follow the zero-shot user rating prediction in~\cite{kang2023llms} that provides the user viewing history and ratings as prompt and invokes the API to predict user ratings on candidate items. Since this approach does not allow setting a batch size, the table presents the average response time per sample. For REKA, we evaluate the two acceleration strategies as introduced in Section~\ref{sec:speed_up}: $\textbf{REKA}_{w/\,apt}$, where the adaptor participates in the inference stage, and $\textbf{REKA}_{w/o\,apt}$, where the adaptor is detached from inference. As we have different version of knowledge generation, which also impact the inference speed, we present four variants of REKA in Table~\ref{tab:inference}: $\textbf{REKA-I}_{w/\,apt}$, $\textbf{REKA-I}_{w/o\,apt}$, $\textbf{REKA-C}_{w/\,apt}$, and $\textbf{REKA-C}_{w/o\,apt}$. The experiments of REKA and base model are all conducted on a Tesla V100 with 32G memory, with a batch size of 256. With the same Tesla V100, we also test \textbf{TALLRec} and only showcase the average inference time per sample, since 32G memory cannot handle LLM with batch size of 256. Table~\ref{tab:inference} presents the average inference time, from which we draw the following conclusions.

\begin{table}[h]
\centering
% \vspace{-5pt}
\caption{The comparison of inference time (s).}
% \vspace{-5pt}
\scalebox{1.0}{
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{ccc}
\toprule
\textbf{Model}      & \textbf{MovieLens-1M} & \textbf{Amazon-Books} \\
\midrule
ChatGPT API   & $5.54$ & $4.11$ \\
TALLRec   &  $7.63\times10^{-1}$ & $7.97\times10^{-1}$ \\
% P5   &  &  \\
$\text{REKA-I}_{w/\,\,apt}$  & $8.08\times10^{-2}$ & $9.39\times10^{-2}$ \\

$\text{REKA-C}_{w/\,\,apt}$  & $4.63\times10^{-2}$ & $4.70\times10^{-2}$ \\
$\text{REKA-I}_{w/o\,\,apt}$ & $6.64\times10^{-3}$ & $1.11\times10^{-2}$\\

$\text{REKA-C}_{w/o\,\,apt}$ & $6.56\times10^{-3}$ & $1.11\times10^{-2}$\\
base DIN     & $6.42\times10^{-3}$ & $1.09\times10^{-2}$\\
\bottomrule
\end{tabular}
}}
\vspace{-5pt}
\label{tab:inference}
\end{table}

Firstly, adopting LLM for direct inference is not feasible for RSs due to its large computational latency. The response latency of ChatGPT API is 4-6 seconds, which does not meet the real-time requirement of RSs typically demanding a response latency of within 100ms. Even if we finetune a relatively small LLM, such as TALLRec based on LLaMa2-7B, its inference latency is still close to 1 second, which is unbearable for industrial scenarios. 

Secondly, both acceleration methods of REKA achieve an inference time within 100ms, satisfying the low latency requirement. When using the prestoring knowledge representation approach, $\textbf{REKA-C}_{w/\,apt}$ has a shorter inference time than $\textbf{REKA-I}_{w/o\,apt}$. This is because $\textbf{REKA-C}_{w/o\,apt}$ employs BERT as the encoder, resulting in knowledge representation with a dimension of 768. On the other hand, $\textbf{REKA-I}_{w/o\,apt}$ uses ChatGLM-6B as the encoder, producing representations with a dimension of 4096, which requires more processing time. Importantly, if we employ the approach of prestoring user and item augmented vectors, the knowledge generation method no longer has a significant impact. In other words, the actual inference time of $\text{REKA-I}_{w/o\,apt}$ and  $\text{REKA-C}_{w/o\,apt}$ is becomes nearly identical, almost the same as that of the backbone model. This demonstrates the effectiveness of our proposed REKA and acceleration strategies. 






\subsection{Ablation Study}
\subsubsection{User and Item Knowledge (RQ6)}\label{reas_fact_konwledge}

To study the impact of knowledge generated by LLMs, we conduct an ablation study on user and item knowledge on the Amazon-Books dataset. 
The two knowledge generation approaches, individual knowledge extraction (REKA-I) and collective knowledge extraction (REKA-C), both produce user and item knowledge, so here we use REKA-I as an example.
% Since the collective knowledge generated by REKA-C all involves reasoning ability of LLMs, the boundaries between reasoning and factual knowledge are not clear. Therefore, this experiment is based on REKA-I, where we consider the knowledge generated for items as factual knowledge and for users as reasoning knowledge.
We select DCNv2, AutoInt, and DIN as backbone models and compare their performance with different knowledge enhancements, as shown in Figure~\ref{fig:knowledge_abaltion}. The legend \textbf{``None"} represents the backbone model without any knowledge enhancement. \textbf{``Item"} and \textbf{``User"} indicate the backbone models enhanced with item knowledge and user knowledge, respectively, while \textbf{``Both"} represents the joint use of both knowledge types.

\begin{figure}[h]
    \centering
% \vspace{-7pt}
    \includegraphics[width=0.65\textwidth]{imgs/knowledge6.pdf}
% \vspace{-6pt}
    \caption{Ablation study about user and item knowledge on Amazon-Books dataset.}
\vspace{-5pt}
    \label{fig:knowledge_abaltion}
\end{figure}

From Figure~\ref{fig:knowledge_abaltion}, we observe that both item knowledge and user knowledge can improve the performance of backbone models, with user knowledge exhibiting a larger improvement. This could be attributed to the fact that user knowledge inferred by the LLMs captures in-depth user preferences, thus compensating for the backbone model's limitations in reasoning underlying motives and intentions. Additionally, the joint use of both user and item enhancements outperforms using either one alone, even achieving a synergistic effect where $1+1>2$. One possible explanation is that user knowledge contains external information that is not explicitly present in the raw data. When used independently, this external knowledge could not be matched with candidate items. However, combining the externally generated item factual knowledge from the LLMs aligned with user knowledge allows RSs to gain a better understanding of items according to user preferences.

\begin{table}[h]
\centering
% \vspace{-7pt}
\caption{Impact of different knowledge encoders. 
% LL is short for LogLoss.
% \Jianghao{The best results are given in bold, while the second-best values are underlined.}
}
% \vspace{-7pt}
\scalebox{1.0}{
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{ccccc|cccc}
\toprule
\multirow{3}{*}{\textbf{Variants}} & \multicolumn{4}{c|}{\textbf{MoiveLens-1M}} & \multicolumn{4}{c}{\textbf{Amazon-Books}} \\
\cmidrule{2-9}
 & \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c|}{\textbf{ChatGLM}} & \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{ChatGLM}} \\
 \cmidrule{2-9}
 & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} \\
 \midrule
base(DIN) & 0.7863 & 0.5486 & 0.7863 & 0.5486 & 0.8304 & 0.4937 & 0.8304 & 0.4937 \\
REKA(LR) & 0.7589 & 0.5811 & 0.7720 & 0.5674 & 0.7375 & 0.5861 & 0.7560 & 0.5718 \\
REKA(MLP) & 0.7754 & 0.5588 & 0.7816 & 0.5559 & 0.7424 & 0.5834 & 0.7571 & 0.5763 \\
REKA-MLP & 0.7934 & 0.5411 & 0.7939 & 0.5401 & 0.8357 & 0.4880 & 0.8370 & 0.4843 \\
REKA-MoE & {\underline{0.7946}} & \textbf{0.5391} & {\underline{0.7950}} & {\underline{0.5394}} & {\underline{0.8371}} & \textbf{0.4841} & {\underline{0.8388}} & {\underline{0.4823}} \\
REKA & \textbf{0.7947} & {\underline{0.5402}} & \textbf{0.7961} & \textbf{0.5370} & \textbf{0.8374} & {\underline{0.4843}} & \textbf{0.8418} & \textbf{0.4801}
\\
\bottomrule
\end{tabular}
}}
% \Jianghao{(1) underline the second best value. (2) significant test is needed}
% \vspace{-10pt}
\label{tab:text_encoder}
\end{table}

% \begin{table}[h]
% \centering
% % \vspace{-7pt}
% \caption{Impact of different knowledge encoders on MoiveLens-1M dataset. 
% % LL is short for LogLoss.
% % \Jianghao{The best results are given in bold, while the second-best values are underlined.}
% }
% % \vspace{-5pt}
% \scalebox{1.2}{
% \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{ccc|cc}
% \toprule
% \multirow{2}{*}{\textbf{Variants}}  & \multicolumn{2}{c|}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{ChatGLM}} \\
%  \cmidrule{2-5}
%  & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} \\
%  \midrule
% % base(DIN) & 0.7975 & 0.5387 & 0.7975 & 0.5387  \\
% % REKA(LR) & 0.7746 & 0.5699 & 0.7903 & 0.5490  \\
% % REKA(MLP) & 0.7882 & 0.5518 & 0.7986 & 0.5399 \\
% % REKA-MLP & {\underline{0.8040}} & 0.5345 & 0.8042 & 0.5318  \\
% % REKA-MoE & \textbf{0.8046} & \textbf{0.5322} & {\underline{0.8052}} & {\underline{0.5305}}  \\
% % REKA & \textbf{0.8046} & {\underline{0.5324}} & \textbf{0.8066} & \textbf{0.5304} \\
% base(DIN) & 0.7863 & 0.5486 & 0.7863 & 0.5486 \\
% REKA(LR) & 0.7589 & 0.5811 & 0.7720 & 0.5674 \\
% REKA(MLP) & 0.7754 & 0.5588 & 0.7816 & 0.5559 \\
% REKA-MLP & 0.7934 & 0.5411 & 0.7939 & 0.5401 \\
% REKA-MoE & \underline{0.7946} & \textbf{0.5391} & \underline{0.7950} & \underline{0.5394} \\
% REKA & \textbf{0.7947} & \underline{0.5402} & \textbf{0.7961} & \textbf{0.5370} \\
% \bottomrule
% \end{tabular}
% }}
% % \Jianghao{(1) underline the second best value. (2) significant test is needed}
% % \vspace{-5pt}
% \label{tab:text_encoder_ml}
% \end{table}

% \begin{table}[h]
% \centering
% % \vspace{-7pt}
% \caption{Impact of different knowledge encoders on Amazon-Books dataset. 
% % LL is short for LogLoss.
% % \Jianghao{The best results are given in bold, while the second-best values are underlined.}
% }
% % \vspace{-5pt}
% \scalebox{1.2}{
% \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{ccc|cc}
% \toprule
% \multirow{2}{*}{\textbf{Variants}} & \multicolumn{2}{c|}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{ChatGLM}}  \\
%  \cmidrule{2-5}
%  & \textbf{AUC} & \textbf{LogLoss} & \textbf{AUC} & \textbf{LogLoss} \\
%  \midrule
% base(DIN) & 0.8304 & 0.4937 & 0.8304 & 0.4937 \\
% REKA(LR)  & 0.7375 & 0.5861 & 0.7560 & 0.5718 \\
% REKA(MLP)  & 0.7424 & 0.5834 & 0.7571 & 0.5763 \\
% REKA-MLP & 0.8357 & 0.4880 & 0.8370 & 0.4843 \\
% REKA-MoE & {\underline{0.8371}} & \textbf{0.4841} & {\underline{0.8388}} & {\underline{0.4823}} \\
% REKA & \textbf{0.8374} & {\underline{0.4843}} & \textbf{0.8418} & \textbf{0.4801}\\
% \bottomrule
% \end{tabular}
% }}
% % \Jianghao{(1) underline the second best value. (2) significant test is needed}
% % \vspace{-5pt}
% \label{tab:text_encoder_amz}
% \end{table}

\subsubsection{Knowledge Encoders and Semantic Transformation (RQ7)}\label{sec:knowledge_encoder}
We employ two different language models, BERT~\cite{bert} and ChatGLM~\cite{du2022glm}, to investigate the impact of different knowledge encoders on \textbf{REKA-I}'s performance. Additionally, we design several variants to demonstrate how the representations generated by knowledge encoders are utilized. \textbf{REKA(LR)} applies average pooling to token representations from the knowledge encoder and directly feeds the result into a linear layer to obtain prediction scores, without utilizing a backbone CTR model. \textbf{REKA(MLP)} replaces the linear layer of REKA(LR) with an MLP. \textbf{REKA-MLP} and \textbf{REKA-MoE} replace the hybrid-expert adaptor with an MLP and a Mixture-of-Experts (MoE), respectively. The original REKA and the two variants, REKA-MLP and REKA-MoE, all adopt DIN as the backbone model. Table~\ref{tab:text_encoder} presents their performance, from which we draw the following conclusions. 

Firstly, we can observe that, overall, variants with ChatGLM as the knowledge encoder outperform those with BERT. The performance of REKA(LR) and REKA(MLP) can be considered as a measure of the quality of the encoded representations, since they directly adopt the representations for prediction. Considering REKA(LR) and REKA(MLP), 
the superior performance of ChatGLM over BERT indicates that ChatGLM performs better in preserving the information within knowledge from LLMs, which may be attributed to the larger size and better text comprehension of ChatGLM (6 billion) compared to BERT (110 million). With ChatGLM on MovieLens-1M, REKA(MLP) is even close to base(DIN), validating the effectiveness of our generated open-world knowledge.


% Since REKA(LR) and REKA(MLP) only utilize the knowledge representations from knowledge encoder, their results can be considered as a measure of the information contained in the representations. On the two variants, 

% Secondly, only leveraging the open-world knowledge generated by LLMs for recommendation can lead to some improvements in certain cases, yet integrating it with recommendation domain knowledge yields more promising results. Among the methods directly utilizing encoded representations, only REKA(MLP) with ChatGLM gains a modest improvement (0.14\% in AUC) over the base(DIN) on MovieLens-1M. However, combining the generated open-world knowledge with the domain knowledge in the classical RSs, as in REKA, brings significant enhancements (1.15\% and 1.38\% AUC improvement) on two datasets. We attribute this improvement to REKA successfully bridging the open-world knowledge and the recommendation domain knowledge.


Secondly, the performance of REKA benefits from complex semantic transformation structures, but the knowledge encoder also limits it. The results on ChatGLM show that a simple MLP is less effective than MoE and our designed hybrid-expert adaptor outperforms the MoE, indicating that the transformation from semantic space to recommendation space entails a complex network structure. However, with BERT as knowledge encoder, REKA-MoE and REKA-MLP exhibit similar performance, suggesting that information from BERT is limited and using an MoE is sufficient in this case.
% \begin{table}[h]
% \centering
% \vspace{-5pt}
% \caption{Impact of different aggregation  and semantic transformation approaches.
% % \Jianghao{The best results are given in bold, while the second-best values are underlined.}
% }
% \vspace{-8pt}
% \scalebox{0.95}{
% \setlength{\tabcolsep}{1.0mm}{
% \begin{tabular}{ccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Variant}} & \multicolumn{2}{c}{\textbf{DIN}} & \multicolumn{2}{c}{\textbf{DCNv2}} & \multicolumn{2}{c}{\textbf{AutoInt}} \\
% \cmidrule{2-7}
%  & \textbf{AUC} & \textbf{Logloss} & \textbf{AUC} & \textbf{Logloss} & \textbf{AUC} & \textbf{Logloss} \\
%  \midrule
%  base     & 0.7975          & 0.5387          & 0.7924 & 0.5451          & 0.7934          & 0.5440          \\
% REKA-last & 0.8037          & 0.5320          & 0.8021 & 0.5346          & 0.8006          & 0.5366          \\
% REKA-wavg & 0.8046          & 0.5335          & 0.8014 & 0.5355          & 0.8023          & 0.5344          \\
% REKA-MLP  & 0.8042          & 0.5318          & 0.8029 & 0.5331          & 0.8031          & 0.5349          \\
% REKA-MoE  & \underline{0.8052}          & \underline{0.5305}          & \underline{0.8036} & \underline{0.5329}          & \underline{0.8041}          & \underline{0.5325}          \\
% REKA      & \textbf{0.8066} & \textbf{0.5304} & \textbf{0.8049} & \textbf{0.5315} & \textbf{0.8060} & \textbf{0.5297} \\
% % base & 0.79748 & 0.53871 & 0.79239 & 0.54508 & 0.79342 & 0.54404 \\
% % REKA-last & 0.80368 & 0.53202 & 0.80208 & 0.53455 & 0.80056 & 0.53658 \\
% % REKA-wavg & 0.80457 & 0.53354 & 0.80138 & 0.53546 & 0.80228 & 0.53440 \\
% % REKA-MLP & 0.80421 & 0.53182 & 0.80293 & 0.53312 & 0.80313 & 0.53485 \\
% % REKA-MoE & 0.80522 & 0.53054 & 0.80355 & 0.53287 & 0.80405 & 0.53249 \\
% % REKA & \textbf{0.80664} & \textbf{0.53037} & \textbf{0.80465} & \textbf{0.53148} & \textbf{0.80601} & \textbf{0.52965} \\
% \bottomrule
% \end{tabular}
% }}
% \label{tab:aggre_transfer}
% % \Jianghao{(1) underline the second best value. (2) significant test is needed}
% \vspace{-8pt}
% \end{table}

% \subsubsection{Aggregation and Semantic Transformation (RQ4)}
% After obtaining representations from knowledge encoder, it is crucial to explore how the aggregation and semantic transformation affect the performance. Therefore, we designed several variants with different aggregation and semantic transformation approaches to investigate their impact. In the original version of \textbf{REKA}, the aggregation function is average pooling over representations of all tokens. \textbf{REKA-last} only utilizes the representation corresponding to the last token, while \textbf{REKA-wavg} applies a weighted average over all the tokens, with higher weights assigned to tokens towards the end of the sequence. Similar to Section~\ref{sec:knowledge_encoder}, \textbf{REKA-MLP} and \textbf{REKA-MoE} replace the hybrid-expert adaptor with an MLP and an MoE, respectively. To ensure a fair comparison, all the variants and REKA use ChatGLM as knowledge encoder and DIN/DCNv2/AutoInt as backbone models, and the comparison is presented in Table~\ref{tab:aggre_transfer}.

% First, compared to REKA, the performances of all variants decline to some extent, yet they still exhibit significant improvement over backbone models. This suggests that different aggregation and semantic transformation methods do influence performance, but they are still capable of combining the knowledge from LLMs with RSs. Furthermore, the performance order of REKA, REKA-wavg, and REKA-last indicates that the useful information for RS is distributed across the representation of various tokens and is not biased toward the end of the sentence. Finally, the results of REKA, REKA-MoE, and REKA-MLP across different backbone models also confirm the finding in Section~\ref{sec:knowledge_encoder} that complex transformation structures can better exploit representations generated by the knowledge encoder.
% \vspace{-5pt}

\section{Broader Impact}
When incorporating LLMs into RSs, it is imperative to give serious consideration to privacy and security issues. While LLMs offer remarkable capabilities, they also come with potential risks of compromising user privacy and generating harmful content~\cite{pan2020privacy,Brown2022privacy,weidinger2021ethical}. We also consider these two issues while designing our proposed framework, REKA.

Regarding privacy, REKA leverages LLMs' reasoning ability and factual knowledge without finetuning LLMs, ensuring that LLMs do not retain or remember user-specific data. Besides, while experiments may involve the use of external APIs on public datasets, real-world implementations usually rely on in-house models, \eg, we utilize Huawei's own LLM PanGu\cite{zeng2021pangu} for online A/B test as described in section~\ref{sec:online}, preventing the leakage of user privacy information through external APIs.

Furthermore, compared to methods that directly display LLM-generated content to users~\cite{chatrec,liu2023chatgpt,dai2023uncovering}, REKA takes a  more proactive stance to mitigate concerns about harmful content and hallucination knowledge generated by LLMs. REKA first converts the textual content from LLMs to robust representations and then incorporates those representations into traditional RSs. This integration avoids displaying
harmful or misleading content generated by LLMs while enabling us to utilize filtering mechanisms commonly used in traditional RSs to screen out potential harmful item recommendations.

Through those measures, REKA strives to deliver robust recommendation performance while safeguarding user data privacy and the security of recommendation content. 
% This approach is aimed at maintaining user trust ans ensuring a high-quality personalized recommendation experience.

\section{Conclusion}

Our work presents REKA, a framework for effectively incorporating open-world knowledge into recommender systems by exploiting large language models. REKA identifies two types of critical knowledge from LLMs, the reasoning knowledge on user preferences and factual knowledge on items, which can be proactively acquired by our designed factorization prompting. A hybrid-expert adaptor is devised to transform the obtained knowledge for compatibility with recommendation tasks. The obtained augmented vectors can then be used to enhance the performance of any recommendation model. Additionally, efficient inference is achieved through preprocessing and prestoring the LLM knowledge. REKA shows superior performance compared to the state-of-the-art methods and is compatible with various recommendation algorithms. 
% \Jianghao{maybe we should mention some future works}

% In future work, we plan to explore additional tasks, datasets, and diverse strategies for utilizing augmented features. 
